Hermite coordinate interpolation kernels: application to image zooming

A number of basic image processing tasks, such as any geometric transformation require interpolation at subpixel image values. In this work we utilize the multidimensional coordinate Hermite spline interpolation defined on non-equal spaced, rectilinear grids and apply it to a very common image processing task, image zooming. Since Hermite interpolation utilizes function values, as well as partial derivative values, it is natural to apply it to image processing tasks as a special case of equi-spaced grid, using numerical approximations of the image partial derivatives at each pixel. Furthermore, the task of image interpolation requires the calculation of image values at positions with nono-zero fractional part. Thus, any spline interpolation can be written as convolution with an appropriate kernel. In this context we generate the Hermite kernels according to the derived $n-$dimensional interpolant of Theorem 2 in [1]. We show that despite the increased complexity of the interpolant, once the kernels are constructed, the Hermite spline interpolation can be applied to images as efficiently as any other less complicated method. Finally, we perform illustrative numerical examples to showcase the applicability and high accuracy of the proposed Hermite kernels for image zooming, compared to other interpolation methods, both traditional convolution-based, as well as employing deep learning, in terms of PSNR, as well as SSIM error metrics. The proposed Hermite spline kernels outperform all other methods in the majority of the test images, in experiments using many cascaded repetitions of the zoom operation. Interesting conclusions can be drawn considering all methods under comparison.

==> conc.tex <==
In this work a new derivation of the coordinate Hermite interpolating polynomial, given the values of the function and its partial derivatives on $n$-dimensional non-regular grids has been proposed. The algebraic and computational complexity of the derived formula is significantly lower compared to the only alternative formulation in the literature \cite{fractmult}.
Furthermore, we provided the remainder of the interpolation in integral form, as well as cascaded polynomial divisions, in case of interpolating polynomial functions, using the Gr{\"o}bner basis of the ideal of the interpolation. The proposed interpolant polynomial can be used for accurate interpolation of data in any number of dimensions, with any degree of partial derivatives at the measured data points. A few arithmetic results of analytic functions are provided, demonstrating the superiority of Hermite interpolation in 2 and 3 dimensions, against a number of other interpolation techniques.

Further work includes the computational implementation of the proposed Hermite polynomial formula utilizing appropriate look-up tables foe equidistant grids, that will allow fast applications on interpolating multidimensional signals.

==> error.tex <==
In this section, we derive an expression for the error of the interpolation formula given
in Theorem \ref{finterpform}, which is identical to the error of Theorem \ref{th1}, for the class of real functions   $f\left( x_{1},\dots,x_{n}\right) $, which can be continued  analytically as a
single valued, regular function $f\left( z_{1},\dots,z_{n}\right) $ of $n$
complex variables in a certain cross-product region $D_{z_{1}}\times
\dots \times D_{z_{n}}$.

In the case of a single variable $x$, let $C$ be a closed contour
in the region $D_{z}$ of analytic continuation of a real function $f(x)$
containing the points $a\in A$ in its interior. Let as denote 
\begin{equation*}
H\left( x\right) =\prod_{a\in A}\left( x-{a}\right) ^{\nu \left( a\right) }.
\end{equation*}

By applying the residue theorem to the contour integral  
\begin{equation*}
\frac{1}{2\pi i}\int_{C}\frac{f\left( z\right) }{\left( z-x\right) H\left(
z\right) }dz,
\end{equation*}%
we obtain (see \cite{GHITV}) 
\begin{equation}\label{fpxint1}
f(x)=p\left( x\right) +\frac{H\left( x\right) }{2\pi i}\int_{C}\frac{f\left(
z\right) }{\left( z-x\right) H\left( z\right) }dz,
\end{equation}%
where 
\begin{equation*}
p\left( x\right) =\sum_{a\in A}\sum_{k=0}^{\nu \left( a\right) -1}f^{\left(
k\right) }\left( a\right) H_{a}^{k},
\end{equation*}

From (\ref{fpxint1}) we have 
\begin{equation*}
\frac{1}{2\pi i}\int_{C}\frac{f\left( z\right) }{z-x}dz=p\left( x\right) -%
\frac{H\left( x\right) }{2\pi i}\int_{C}\frac{f\left( z\right) }{\left(
z-x\right) H\left( z\right) }dz,
\end{equation*}%
or equivalently 
\begin{equation}\label{fp1}
\frac{1}{2\pi i}\int_{C}\frac{H\left( z\right) -H\left( x\right) }{H\left(
z\right) \left( z-x\right) }f\left( z\right) dz=p\left( x\right).
\end{equation}

In the following, we assume that $C_{j},\;j=1,\dots,n$ are simple closed contours in the
regions $D_{j}$  containing $A_{j}$ in their
interior, of analyticity of $f\left(x_{1},\dots,x_{j-1},z_{j},x_{j+1},\dots,x_{n}\right) $, where $x_{1},\dots,x_{j-1},x_{j+1},\dots,x_{n}$ are fixed. Further, we assume that $f\left( z_{1},\dots,z_{n}\right) $ is
simultaneously analytic in $D_{z_{1}}\times \dots\times D_{z_{n}}$.

Finally, we introduce the following notation: 
\begin{equation*}
H_r (w_r) = \prod_{a\in A_r} (w_r -a)^{\nu_r (a)},\; r=1,\dots, n.
\end{equation*}

\begin{lem}\label{lemErr}
The following identity holds:%
\begin{eqnarray}\label{lemrel1}
&&\frac{1}{\left( 2\pi i\right) ^{n}}\int_{C_{1}}\dots\int_{C_{n}}\frac{%
\prod_{r=1}^{n}\left( H_{r}\left( z_{r}\right) -H_{r}\left( x_{r}\right)
\right) }{\prod_{r=1}^{n}\left( z_{r}-x_{r}\right) H_{r}\left( z_{r}\right) }%
f\left( z_{1},\dots,z_{n}\right) dz_{1}\dots dz_{n} =\sum_{\mathbf{a\in A}}\sum_{\mathbf{k\in }\left[ \mathbf{0,}\nu \left( 
\mathbf{a}\right) -\mathbf{1}\right] }H_{\mathbf{a}}^{\mathbf{k}}\partial _{%
\mathbf{a}}^{\mathbf{k}}f.  
\end{eqnarray}
\end{lem}

\begin{proof}
We will prove by induction with respect to $n$: For $n=1$, (\ref{lemrel1}) reduces to (\ref{fpxint1}). Let (\ref{lemrel1}) hold for $n-1$. Then 
\begin{eqnarray*}
&&\frac{1}{\left( 2\pi i\right) ^{n}}\int_{C_{1}}\dots\int_{C_{n}}\frac{%
\prod_{r=1}^{n}\left( H_{r}\left( z_{r}\right) -H_{r}\left( x_{r}\right)
\right) }{\prod_{r=1}^{n}\left( z_{r}-x_{r}\right) H_{r}\left( z_{r}\right) }%
f\left( z_{1},\dots,z_{n}\right) dz_{1}\dots dz_{n} \\
&=&\frac{1}{2\pi i}\int_{C_{n}}\frac{H_{n}\left( z_{n}\right) -H_{n}\left(
x_{n}\right) }{\left( z_{n}-x_{n}\right) H_{n}\left( z_{r}\right) }\left( 
\frac{1}{\left( 2\pi i\right) ^{n-1}}\int_{C_{1}}\dots\int_{C_{n-1}}\frac{%
\prod_{r=1}^{n-1}\left( H_{r}\left( z_{r}\right) -H_{r}\left( x_{r}\right)
\right) }{\prod_{r=1}^{n-1}\left( z_{r}-x_{r}\right) H_{r}\left(
z_{r}\right) }f\left( z_{1},\dots,z_{n}\right) dz_{1}\dots dz_{n-1}\right) dz_{n}
\\
&=&\frac{1}{2\pi i}\int_{C_{n}}\frac{H_{n}\left( z_{n}\right) -H_{n}\left(
x_{n}\right) }{\left( z_{n}-x_{n}\right) H_{n}\left( z_{r}\right) }%
\sum_{a_{n}\in A_{1}}\dots\sum_{a_{n}\in A_{n}}\sum_{k_{1}=0}^{\nu _{1}\left(
a_{1}\right) -1}\dots\sum_{k_{n-1}=0}^{\nu _{n-1}\left( a_{n-1}\right)
-1}\prod_{j=1}^{n-1}H_{a_{j}}^{k_{j}}\left( x_{j}\right) \frac{\partial ^{%
%\NEG
{k}_{1}+\dots+k_{n-1}}}{\partial x_{1}^{k_{1}}\dots \partial x_{n-1}^{k_{n-1}}%
}f\left( a_{1,}\dots, a_{n-1},z_{n}\right) dz_{n}\\
&=& \sum_{a_{n}\in A_{1}}\dots\sum_{a_{n}\in A_{n}}\sum_{k_{1}=0}^{\nu _{1}\left(
a_{1}\right) -1}\dots\sum_{k_{n-1}=0}^{\nu _{n-1}\left( a_{n-1}\right)
-1}\prod_{j=1}^{n-1} H_{a_{j}}^{k_{j}}(x_j)\left( \frac{1}{2\pi i} \int_{C_{n}}\frac{H_{n}\left( z_{n}\right) -H_{n}\left(
x_{n}\right) }{\left( z_{n}-x_{n}\right) H_{n}\left( z_{r}\right) }  \frac{\partial ^{%
%\NEG
{k}_{1}+\dots+k_{n-1}}}{\partial x_{1}^{k_{1}}\dots \partial x_{n-1}^{k_{n-1}}%
}f\left( a_{1,}\dots, a_{n-1},z_{n}\right) dz_{n}  \right) 
.
\end{eqnarray*}%
Thus, using (\ref{fp1}) we obtain:  
\begin{eqnarray*}
&&\frac{1}{\left( 2\pi i\right) ^{n}}\int_{C_{1}}\dots\int_{C_{n}}\frac{%
\prod_{r=1}^{n}\left( H_{r}\left( z_{r}\right) -H_{r}\left( x_{r}\right)
\right) }{\prod_{r=1}^{n}\left( z_{r}-x_{r}\right) H_{r}\left( z_{r}\right) }%
f\left( z_{1},\dots,z_{n}\right) dz_{1}\dots dz_{n} \\
&=&\sum_{a_{1}\in A_{1}}\dots\sum_{a_{n}\in A_{n}}\sum_{k_{n}=0}^{\nu
_{1}\left( a_{1}\right) -1}\dots \sum_{k_{n}=0}^{\nu _{n}\left( a_{n}\right)
-1}\ \prod_{j=1}^{n}H_{a_{j}}^{k_{j}}\left( x_{j}\right) \frac{\partial ^{%
%\NEG
{k}_{n}+\dots+k_{1}}}{\partial x_{n}^{k_{n}}\dots\partial x_{1}^{k_{1}}}%
f\left( a_{1},\dots, a_{n}\right) \\
&=&\sum_{\mathbf{a\in A}}\sum_{\mathbf{k\in }\left[ \mathbf{0,}\nu \left( 
\mathbf{a}\right) -\mathbf{1}\right] }H_{\mathbf{a}}^{\mathbf{k}}\partial _{%
\mathbf{a}}^{\mathbf{k}}f.
\end{eqnarray*}
\end{proof}

The interpolation error is derived in the following Theorem.
\begin{thm}\label{errform}
The error of the interpolation formula of Theorem \ref{finterpform} is defined as
\begin{equation*}
R:=f-\sum_{\mathbf{a\in A}}\sum_{\mathbf{k\in }\left[ \mathbf{0,}\nu \left( 
\mathbf{a}\right) -\mathbf{1}\right] }t_{\mathbf{a}}^{\mathbf{k}}H_{\mathbf{a%
}}^{k},
\end{equation*}%
where $t_{\mathbf{a}}^{\mathbf{k}}=\partial _{\mathbf{a}}^{\mathbf{k}}f$ ,
 is given by:
\begin{equation}\label{211}
R=\frac{1}{\left( 2\pi i\right) ^{n}}\int_{C_{1}}\dots \int_{C_{n}}\frac{%
\prod_{r=1}^{n}H_{r}\left( z_{r}\right) -\prod_{r=1}^{n}\left( H_{r}\left(
z_{r}\right) -H_{r}\left( x_{r}\right) \right) }{\prod_{r=1}^{n}\left(
z_{r}-x_{r}\right) H_{r}\left( z_{r}\right) }f\left( z_{1},\dots,z_{n}\right)
dz_{1}\dots dz_{n}. 
\end{equation}
\end{thm}

\begin{proof}
From (\ref{lemrel1}) we have
\begin{eqnarray}\label{212}
&&\frac{1}{\left( 2\pi i\right) ^{n}}\int_{C_{1}}\dots\int_{C_{n}}\frac{%
\prod_{r=1}^{n}H_{r}\left( z_{r}\right) -\prod_{r=1}^{n}\left( H_{r}\left(
z_{r}\right) -H_{r}\left( x_{r}\right) \right) }{\prod_{r=1}^{n}\left(
z_{r}-x_{r}\right) H_{r}\left( z_{r}\right) }f\left( z_{1},\dots,z_{n}\right)
dz_{1}\dots dz_{n}  \\
&=&\frac{1}{\left( 2\pi i\right) ^{n}}\int_{C_{1}}\dots\int_{C_{n}}\frac{1}{%
\prod_{r=1}^{n}\left( z_{r}-x_{r}\right) }f\left(
z_{1},\dots,z_{n}\right) dz_{1}\dots dz_{n}-\sum_{\mathbf{a\in A}}\sum_{\mathbf{%
k\in }\left[ \mathbf{0,}\nu \left( \mathbf{a}\right) -\mathbf{1}\right] }H_{%
\mathbf{a}}^{\mathbf{k}}\partial _{\mathbf{a}}^{\mathbf{k}}f \nonumber.
\end{eqnarray}

By applying the residue Theorem $n$-times, we obtain%
\begin{equation}\label{213}
\frac{1}{\left( 2\pi i\right) ^{n}}\int_{C_{1}}\dots\int_{C_{n}}\frac{1}{%
\prod_{r=1}^{n}\left( z_{r}-x_{r}\right) }f\left(
z_{1},\dots,z_{n}\right) dz_{1}\dots dz_{n}=f\left( x_{1},\dots,x_{n}\right) . 
\end{equation}%
From relations (\ref{212}) and (\ref{213}) we get (\ref{211}).
\end{proof}

\begin{rem}
{\rm
Applying Theorem \ref{errform} for $n=2$ we obtain the error formula for the bivariate Hermite polynomial, as given in \cite[Section 5]{GHITV}.
}
\end{rem}

\begin{rem}
{\rm
Lemma \ref{lemErr} provides an alternative way of generating the Hermite polynomial that interpolates any function $f$, provided that the integral can be calculated. %\textcolor{red}{A relevant example will be given in the next section.}
}
\end{rem}

\begin{rem}
{\rm
Lemma \ref{lemErr} and Theorem \ref{errform} hold also for complex functions of complex variables and for finite subsets $A_1,\dots ,A_n$ of $\mathbb{C}$.}
\end{rem}

\begin{rem}\label{rem8}
{\rm
Let us denote by $H\left( D_{z_{1}}\times \dots \times D_{z_{n}}\right) $ the
ring of all holomorphic functions on $D_{z_{1}}\times \dots\times D_{z_{n}}$
and by $\left( H_{1},\dots,H_{n}\right) $ the ideal generated by the
polynomials $H_{1},\dots,H_{n}$. Consider the linear operator $T_{\left( 
\mathbf{A,}\nu \right) }:H\left( D_{z_{1}}\times \dots \times D_{z_{n}}\right)
\rightarrow $ $V\left( \mathbf{A,}\nu \right) $ given by 
\begin{equation*}
T_{\left( \mathbf{A,}\nu \right) }\left( f\right) =\frac{1}{\left( 2\pi
i\right) ^{n}}\int_{C_{1}}\dots\int_{C_{n}}\frac{\prod_{r=1}^{n}\left(
H_{r}\left( z_{r}\right) -H_{r}\left( x_{r}\right) \right) }{%
\prod_{r=1}^{n}\left( z_{r}-x_{r}\right) H_{r}\left( z_{r}\right) }f\left(
z_{1},\dots,z_{n}\right) dz_{1}\dots dz_{n}.
\end{equation*}%
Clearly by Lemma
\ref{lemErr} we have that $T_{\left( \mathbf{A,}\nu \right) }$ is an
epimorphism and \begin{equation*}
\ker T_{\left( \mathbf{A,}\nu \right) }=\left\{ g\in
H\left( D_{z_{1}}\times \dots \times D_{z_{n}}\right):\,\partial _{\mathbf{a}}^{\mathbf{m}%
}g=0,~\mathbf{a\in A},~\mathbf{m\in }\left[ \mathbf{0,}\nu \left( \mathbf{a}%
\right) -\mathbf{1}\right] \right\} .
\end{equation*}
By using Leibniz derivative rule for
multivariable functions we have that for any $f\in H\left( D_{z_{1}}\times
\dots\times D_{z_{n}}\right) $ and any $g\in \ker T_{\left( \mathbf{A,}\nu
\right) }$ hold $\partial _{\mathbf{a}}^{\mathbf{m}}(fg)=0$. Therefore $\ker
T_{\left( \mathbf{A,}\nu \right) }$ is an ideal of $H\left( D_{z_{1}}\times
\dots\times D_{z_{n}}\right)$. In other words, $T_{\left( \mathbf{A,}\nu
\right) }$ is an ideal projector. Further by residue Theorem we get $
T_{\left( \mathbf{A,}\nu \right) }\left( H_{r}\right) =0,$ $r=1,\dots,n$ .
Therefore $\left( H_{1},\dots,H_{n}\right) \subseteq \ker T_{\left( \mathbf{A,}
\nu \right) }$.
}
\end{rem}

 In the next section the
connection between the ideals $\left( H_{1},\dots,H_{n}\right) $ and $\ker
T_{\left( \mathbf{A,}\nu \right) }$ will also be determined for any infinite field.


==> examp.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{exam}
{\rm
Consider the grid $\mathbf{A}=A_1 \times A_2$, where $A_1 = \{0,1\},\; A_2 = \{0,1\}$, with multiplicity function $v(a) = (v_1(a),\;v_2(a)) = (2,2)$, for every point on the grid, $a \in \mathbb{A}$. Given the values of the interpolating polynomial $f$, $t_{\mathbf{a}%
}^{\mathbf{k}},~\mathbf{a\in A},~\mathbf{k\in }\left[ \mathbf{0,}\nu \left( 
\mathbf{a}\right) -\mathbf{1}\right] $, namely $t_{(0,0)}^{(0,0)},t_{(1,0)}^{(0,0)},t_{(0,1)}^{(0,0)},t_{(1,1)}^{(0,0)}$ at each one of the support points, as well as the values of the partial derivatives up to the 1st degree: $t_{(0,0)}^{(0,1)},t_{(1,0)}^{(0,1)},t_{(0,1)}^{(0,1)},t_{(1,1)}^{(0,1)}$, $t_{(0,0)}^{(1,0)},t_{(1,0)}^{(1,0)},t_{(0,1)}^{(1,0)},t_{(1,1)}^{(1,0)}$, $t_{(0,0)}^{(1,1)},t_{(1,0)}^{(1,1)},t_{(0,1)}^{(1,1)},t_{(1,1)}^{(1,1)}$, the following conditions must hold: 
$$\partial _{\mathbf{a}}^{\mathbf{k}}f=t_{\mathbf{a}%
}^{\mathbf{k}},~\mathbf{a\in A},~\mathbf{k\in }\left[ \mathbf{0,}\nu \left( 
\mathbf{a}\right) -\mathbf{1}\right].$$

We compute the $H_{\left( i,a\right) }\left( x_{i}\right) $ quantities given by (\ref{Hmikra}) for $i\in \left\{ 1,2\right\} $ and $a\in A_{i}$:
\begin{eqnarray*}
&H_{(1,0)} =x_1^2 - 2x_1+1&,H_{(2,0)} = x_2^2 -2x_2 + 1\\ &H_{(1,1)}=x_1^2&, H_{(2,1)} = x_2^2
\end{eqnarray*}

Furthermore, we compute the $H_{(\mathbf{a},\mathbf{k})}$ quantities  given by (\ref{Hmegala}) for every $\mathbf{a} \in \mathbf{A}$ and $\mathbf{k} \in [\mathbf{0},v(\mathbf{a})-\mathbf{1}]$. The numbering of the elements of $[\mathbf{0},v(\mathbf{a})-\mathbf{1}]$ is given by the degree reverse lexicographic order. More specifically, $$
1_{\mathbf{a}} =\left( 0,0\right) \prec 2_{\mathbf{a}}=\left(
0,1\right) \prec 3_{\mathbf{a}}=\left(1,0\right)\prec  4_{\mathbf{a}} =\left( 1,1\right).$$
\begin{eqnarray*}
&H_{(0,0),(0,0)}= (x_1^2 - 2x_1+1)(x_2^2 - 2x_2+1)&, H_{(0,1),(0,0)}= (x_1^2 - 2x_1+1)x_2^2\\ 
&H_{(0,0),(0,1)}= (x_1^2 - 2x_1+1)(x_2^3 - 2x_2^2+x_2)&,
H_{(0,1),(0,1)}= (x_1^2 - 2x_1+1)(x_2^3-x^2)\\
&H_{(0,0),(1,0)}= (x_1^3 - 2x_1^2+x_1)(x_2^2 - 2x_2+1)&,
H_{(0,1),(1,0)}= (x_1^3 - 2x_1^2+x_1)x_2^2\\
&H_{(0,0),(1,1)}= (x_1^3 - 2x_1^2+x_1)(x_2^3 - 2x_2^2+x_2)&,
H_{(0,1),(1,1)}= (x_1^3 - 2x_1^2+x_1)(x_2^3-x^2)\\
\\
&H_{(1,0),(0,0)}= x_1^2(x_2^2 - 2x_2+1)&,
H_{(1,1),(0,0)}= x_1^2x_2^2\\
&H_{(1,0),(0,1)}= x_1^2(x_2^3 - 2x_2^2+x_2)&,
H_{(1,1),(0, 1)}=x_1^2(x_2^3-x_2^2)\\
&H_{(1,0),(1,0)}=(x_1^3-x_1^2)(x_2^2 - 2x_2+1)&,
H_{(1,1),(1,0)}= (x_1^3-x_1^2)x_2^2\\
&H_{(1,0),(1,1)}= (x_1^3-x_1^2)(x_2^3 - 2x_2^2+x_2)&,
H_{(1,1),(1,1)}= (x_1^3-x_1^2)(x_2^3-x_2^2)\\
\end{eqnarray*}

Thus, $H_{{(0,0)}}=\left(H_{(0,0),(0,0)},\; H_{(0,0),(0,1)},\; H_{(0,0),(1,0)},\; H_{(0,0),(1,1)} \right)^T$. Similarly, for $H_{{(0,1)}},\; H_{{(1,0)}}$ and $H_{{(1,1)}}$.

For  each point on the grid, we create the lower triangular matrix, $L_{\mathbf{a}}$:
\begin{eqnarray*}
    \Lambda_{(0,0)}^{-1} =
    \left(  
    \begin{array}{cccc}
    1 &  0 & 0 & 0 \\
    -2 & 1 & 0 & 0 \\
    -2 & 0 & 1 & 0 \\
    4 & -2 & -2 & 1
    \end{array}   
    \right)&,&
        \Lambda_{(0,1)}^{-1} =
    \left(  
    \begin{array}{cccc}
    1 &  0 & 0 & 0 \\
    2 & 1 & 0 & 0 \\
    -2 & 0 & 1 & 0 \\
    -4 & -2 & 2 & 1
    \end{array}   
    \right),\\
    \\
    \Lambda_{(1,0)}^{-1} =
    \left(  
    \begin{array}{cccc}
    1 &  0 & 0 & 0 \\
    -2 & 1 & 0 & 0 \\
    2 & 0 & 1 & 0 \\
    -4 & 2 & -2 & 1
    \end{array}   
    \right)&,&
        \Lambda_{(1,1)}^{-1} =
    \left(  
    \begin{array}{cccc}
    1 &  0 & 0 & 0 \\
    2 & 1 & 0 & 0 \\
    2 & 0 & 1 & 0 \\
    4 & 2 & 2 & 1
    \end{array}   
    \right),
\end{eqnarray*}

The interpolating polynomial obtained by using the formula of Theorem \ref{finterpform} is
\begin{eqnarray}\label{exampinterpol}
     f &=& \left(  \Lambda_{(0,0)}^{-1} \cdot
    \left(  
    \begin{array}{c}
    t_{(0,0)}^{(0,0)} \\
    t_{(0,0)}^{(0,1)}  \\
    t_{(0,0)}^{(1,0)}  \\
    t_{(0,0)}^{(1,1)} 
    \end{array}   
    \right)\right)^T
     \left(  
    \begin{array}{c}
    H_{(0,0),(0,0)} \\
    H_{(0,0),(0,1)}  \\
    H_{(0,0),(1,0)} \\
    H_{(0,0),(1,1)} 
    \end{array}   
    \right) 
    +
    \left(  \Lambda_{(0,1)}^{-1} \cdot
    \left(  
    \begin{array}{c}
    t_{(0,1)}^{(0,0)} \\
    t_{(0,1)}^{(0,1)}  \\
    t_{(0,1)}^{(1,0)}  \\
    t_{(0,1)}^{(1,1)} 
    \end{array}   
    \right)\right)^T
     \left(  
    \begin{array}{c}
    H_{(0,1),(0,0)} \\
    H_{(0,1),(0,1)}  \\
    H_{(0,1),(1,0)} \\
    H_{(0,1),(1,1)} 
    \end{array}   
    \right) \nonumber\\
    &+&
    \left(  \Lambda_{(1,0)}^{-1} \cdot
    \left(  
    \begin{array}{c}
    t_{(1,0)}^{(0,0)} \\
    t_{(1,0)}^{(0,1)}  \\
    t_{(1,0)}^{(1,0)}  \\
    t_{(1,0)}^{(1,1)} 
    \end{array}   
    \right)\right)^T
     \left(  
    \begin{array}{c}
    H_{(1,0),(0,0)} \\
    H_{(1,0),(0,1)}  \\
    H_{(1,0),(1,0)} \\
    H_{(1,0),(1,1)} 
    \end{array}   
    \right) 
    +
    \left(  \Lambda_{(1,1)}^{-1} \cdot
    \left(  
    \begin{array}{c}
    t_{(1,1)}^{(0,0)} \\
    t_{(1,1)}^{(0,1)}  \\
    t_{(1,1)}^{(1,0)}  \\
    t_{(1,1)}^{(1,1)} 
    \end{array}   
    \right)\right)^T
     \left(  
    \begin{array}{c}
    H_{(1,1),(0,0)} \\
    H_{(1,1),(0,1)}  \\
    H_{(1,1),(1,0)} \\
    H_{(1,1),(1,1)} 
    \end{array}   
    \right) .
\end{eqnarray}
}
\end{exam}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{exam}
{\rm
Let us expand the previous example by using the proposed Hermite polynomial in order to interpolate a given function $g(x_1,x_2) = e^{x_1+x_2}$. To this end, it is sufficient to 
set the values of $t_{ij}^{(km)}$ equal to $\partial_{ij}^{(km)}g$. More specifically:

\begin{equation*}
    \left(  
    \begin{array}{c}
    t_{(0,0)}^{(0,0)} \\
    t_{(0,0)}^{(0,1)}  \\
    t_{(0,0)}^{(1,0)}  \\
    t_{(0,0)}^{(1,1)} 
    \end{array}\right) =
        \left(  
    \begin{array}{c}
    1 \\
    1\\
    1\\
    1
    \end{array}\right),
        \left(  
    \begin{array}{c}
    t_{(0,1)}^{(0,0)} \\
    t_{(0,1)}^{(0,1)}  \\
    t_{(0,1)}^{(1,0)}  \\
    t_{(0,1)}^{(1,1)} 
    \end{array}\right)
    =
    \left(  
    \begin{array}{c}
    t_{(1,0)}^{(0,0)} \\
    t_{(1,0)}^{(0,1)}  \\
    t_{(1,0)}^{(1,0)}  \\
    t_{(1,0)}^{(1,1)} 
    \end{array}\right)
    =
        \left(  
    \begin{array}{c}
    e \\
    e\\
    e\\
    e
    \end{array}\right),
        \left(  
    \begin{array}{c}
    t_{(1,1)}^{(0,0)} \\
    t_{(1,1)}^{(0,1)}  \\
    t_{(1,1)}^{(1,0)}  \\
    t_{(1,1)}^{(1,1)} 
    \end{array}\right) =
        \left(  
    \begin{array}{c}
    e^2 \\
    e^2\\
    e^2\\
    e^2
    \end{array}\right).
\end{equation*}
Substituting the values of $t_{ij}^{(km)}$ in (\ref{exampinterpol}) of the previous example and performing some algebra, yields the following Hermite polynomial. 
\begin{equation*}
    f(x_1,x_2)= (1 - x_1(-1 + (5 + e(-2 + x_1) - 3x_1)x_1))(1 + x_2 + (-5 + 2e x_2^2 - (-3 + e)x_2^3)
\end{equation*}
This polynomial is identical with the one obtained by Eq. (\ref{lemrel1}) from Lemma \ref{lemErr}. 

The calculated RMSE between the original function and the interpolated polynomial, in a grid of $11 \times 11$ equally spaced points in $[0,1] \times [0,1]$ is $0.0085$, which suggests a very accurate interpolation.
}
\end{exam}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{exam}\label{examp2d}
{\rm
Consider the function $g(x_1,x_2) = e^{-(x_1 - 3)^2-(x_2 -3)^2} + e^{\frac{-(x_1 - 4)^2-(x_2-4)^2}{5}}$ and the grid of support points $\mathbf{A}=A_1 \times A_2$, where $A_1 = \{0 ,1,2,3,4,5\},\; A_2 = \{0 ,1,2,3,4,5\}$, with multiplicity function (maximum order of derivation -1) $v(\mathbf{a}) = (v_1(a),\;v_2(a))$, for every point on the grid, $a \in \mathbb{A}$. Thus in total  $6\times 6$ support points have been defined.
The 3d plot of the function, $g(x_1,x_2)$ is depicted in Figure \ref{fig1}. In addition, the difference between $g(x_1,x_2)$ and the interpolated function using the proposed Hermit with maximum order of derivative $v(\mathbf{a}) = (v_1(a),\;v_2(a)) = (2,2)$ and the cubic spline interpolation (which was the best performer of the methods under comparison) are shown in Figure   \ref{fisubfig}(a) and (b) respectively. Note the the color scale is identical in all difference images.
\begin{figure}[!h]
     \centering
         \includegraphics[width=9cm]{figy1.png}
         \caption{Function $g(x_1,x_2) = e^{-(x_1 - 3)^2-(x_2 -3)^2} + e^{\frac{-(x_1 - 4)^2-(x_2-4)^2}{5}}$ of Example \ref{examp2d}}
         \label{fig1}
\end{figure}

\begin{figure}[h!]
\centering
\subfigure[]{{\includegraphics[width=0.5\textwidth]{fsc2.png}}}\hfill
\subfigure[]{{\includegraphics[width=0.5\textwidth]{fsc1.png}}}
\caption{The difference between $g(x_1,x_2)$ of Example \ref{examp2d} and the interpolated function using (a) the proposed Hermit with multiplicity function $v(a) = (v_1(a),\;v_2(a)) = (2,2)$ and (b) the cubic spline interpolation. Note the the color scale is identical in all difference images.}
\label{fisubfig}
\end{figure}

In this example we utilize the values of $g$ and its partial derivatives up to maximum order (m.o.) $v(\mathbf{a})-1$ at each support point $\mathbf{a}$, to interpolate the function at $51 \times 51$ equally distributed points in $[0,5] \times [0,5]$. The cubic spline, linear, cubic polynomial and the Hermit Makima interpolation methods are also applied at the same points, using the Matlab implementation. The achieved RMSE by each method is shown in Table \ref{tably1}, calculated at the aforementioned points. These interpolation methods have been used for comparison purposes in the remaining examples.
\begin{table}[h!]
\begin{center}
\caption{The achieved RMSE for the proposed Hermite polynomial and other interpolation methods, in the case of Example \ref{examp2d}}\label{tably1}
\begin{tabular}{|l cc|}
\hline
\textbf{Method} & \textbf{RMSE} &\\ \hline\hline 
Proposed Hermite $v(\mathbf{a}) = (2,2)$ & 0.0054  & \\ \hline
Proposed Hermite $v(\mathbf{a})= (3,3)$ & 0.0002 & \\ \hline
Linear &  0.0554 &  \\ \hline
Cubic   & 0.0237 &  \\ \hline
Makima  & 0.0255 & \\ \hline
Spline  & 0.0223 & \\ \hline
\hline
\end{tabular}
\end{center}
\end{table}

}
\end{exam}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{exam}\label{examp3d}
{\rm
Consider the function $g(x_1,x_2,x_3) = e^{\frac{-(x_1 - 3)^2-(x_2 -1)^2-(x_3 -1.5)^2)}{3}}- e^{\frac{-(x_1 - 0.5)^2-(x_2 -2)^2-(x_3 -1)^2)}{5}}$, and the grid of support points $\mathbf{A}=A_1 \times A_2 \times A_3$, where $A_1 = \{0 ,1,2,3\},\; A_2 = \{0 ,1,2,3,4\}$ and $A_3 = \{0,1,2\}$, with multiplicity function $v(\mathbf{a}) = (v_1(\mathbf{a}),\;v_2(\mathbf{a}),\;v_3(\mathbf{a})) = (1,1,1) , (2,2,2)$ and $(3,3,3)$, for every point on the grid, $\mathbf{a} \in \mathbf{A}$. Thus, in total we utilize $4 \times 5 \times 3$ support points to derive the Hermite interpolating polynomial. 

In this example we use the values of $g$ and its partial derivatives up to maximum order,  $v(\mathbf{a})-1$, at each support point $\mathbf{a}$, to interpolate the function at $13 \times 17 \times 9$ equally distributed points in $[0,3] \times [0,4] \times [0,2]$. The cubic spline, linear, cubic polynomial and the Hermit Makima interpolation methods are also applied at the same points. The achieved RMSE by each method is shown in Table \ref{table2}, calculated at the aforementioned points.

\begin{table}[!h]
\begin{center}
\caption{The achieved RMSE for the proposed Hermite polynomial and other interpolation methods, in the case of Example \ref{examp3d}}\label{table2}
\begin{tabular}{|l cc|}
\hline
Method & RMSE &\\ \hline
Proposed Hermite $v(\mathbf{a}) = (1,1,1)$ & 0.0152  & \\ \hline
Proposed Hermite $v(\mathbf{a}) = (2,2,2)$ &  0.0001 & \\ \hline
Proposed Hermite $v(\mathbf{a}) = (3,3,3)$ & 1.2776e-06 & \\ \hline
Linear &  0.0528 &  \\ \hline
Cubic   & 0.0187 &  \\ \hline
Makima  & 0.0209 & \\ \hline
Spline  & 0.0152 & \\ \hline
\hline
\end{tabular}


\end{center} 
\end{table}
}
\end{exam}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{exam}
{\rm
    Consider the grid $\mathbf{A}=A_1 \times A_2$, where $A_1 = \{0,1\},\; A_2 = \{0,1\}$, with multiplicity function $v(a) = (v_1(a),\;v_2(a)) = (1,1)$, for every point on the grid, $a \in \mathbf{A}$. The given values of the support points are $c_{00}, \; c_{01},\;c_{10},\;c_{11}$, such that $t_{(i,j)}^{(0,0)}=c_{ij}, i,j = \{0,1\}$.

    The expressions $H_{\left( i,a\right) }\left( x_{i}\right) $ in (\ref{Hmikra}) are obtained for $i\in \left\{ 1,2\right\} $ and $a\in A_{i}$ as following:  $H_{(1,0)} =1-x_1,\; H_{(1,1)} =x_1,\; H_{(2,0)} =1-x_2$, and $H_{(2,1)} =x_2$.

    Furthermore, we derive $H_{(\mathbf{a},\mathbf{k})}$ given by (\ref{Hmegala}) for every $\mathbf{a} \in \mathbf{A}$ and $\mathbf{k}=(0,0)$: 
    \begin{eqnarray*}
     H_{(0,0),(0,0)} &=& (1-x_1)(1-x_2) ,\\ H_{(0,1),(0,0)}&=& (1-x_1)x_2,\\ H_{(1,0),(0,0)}&=& x_1(1-x_2), \\ H_{(1,1),(0,0)} &=& x_1x_2.
    \end{eqnarray*}

    Note that for every $\mathbf{a} \in \mathbf{A}$, $\Lambda_{\mathbf{a}}=1$. Thus, the interpolating polynomial is given by the following expression:
    \begin{equation}\label{bil}
        f(x_1,x_2) = c_{00} (1-x_1)(1-x_2)+c_{01}(1-x_1)x_2 + c_{10} x_1(1-x_2)  + c_{11}x_1x_2
    \end{equation}
    
    Observe that the above expression is identical to the bilinear interpolating polynomial for the unit step grid.
    
    %\begin{comment}
    %\begin{tikzpicture}
    %\draw[help lines, %color=gray!30, dashed] %(0,0) grid (2,2);
    %\draw[->,ultra thick] %(-0.1,0)--(2,0) %node[right]{$x_1$};
    %\draw[->,ultra thick] (0,-0.1)--(0,2) node[above]{$x_2$};
    %\end{tikzpicture}
    %\end{comment} 
}
\end{exam}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{exam}
    Consider the grid $\mathbf{A}=A_1 \times A_2 \times A_3$, where $A_1 = \{0,1\},\; A_2 = \{0,1\}, \; A_3 = \{0,1\}$, with multiplicity function $v(a) = (v_1(a),\;v_2(a),\;v_3(a)) = (1,1,1)$, for every point on the grid, $a \in \mathbf{A}$. The given values of the support points are $c_{000},c_{001},c_{010},c_{100},c_{011},c_{101},c_{110},c_{111}$, such that $t_{(i,j,k)}^{(0,0,0)}=c_{ijk}, i,j,k = \{0,1\}$.

    We derive $H_{\left( i,a\right) }\left( x_{i}\right) $  given by (\ref{Hmikra}) for $i\in \left\{ 1,2\right\} $ and $a\in A_{i}$:  $H_{(1,0)} =1-x_1,\; H_{(1,1)} =x_1,\; H_{(2,0)} =1-x_2$,$H_{(2,1)} =x_2, H_{(3,0)} =1-x_3,$ and $\; H_{(1,1)} =x_3$.
    Furthermore, we obtain $H_{(\mathbf{a},\mathbf{k})}$   given by (\ref{Hmegala}) for every $\mathbf{a} \in \mathbf{A}$ and $\mathbf{k}=(0,0,0)$: 
\begin{eqnarray*}
&H_{(0,0,0),(0,0,0)}= (1-x_1)(1-x_2)(1-x_3)&, H_{(0,0,1),(0,0,0)}=  (1-x_1)(1-x_2)x_3\\ 
&H_{(0,1,0),(0,0,0)}=  (1-x_1)x_2(1-x_3)&,
H_{(1,0,0),(0,0,0)}= x_1(1-x_2)(1-x_3)\\
&H_{(0,1,1),(0,0,0)}=(1-x_1)x_2x_3&,
H_{(1,0,1),(0,0,0)}= x_1(1-x_2)x_3\\
&H_{(1,1,0),(0,0,0)}= x_1 x _2 (1-x_3)&,
H_{(1,1,1),(0,0,0)}= x_1 x_2 x_3
\end{eqnarray*}

%For every $\mathbf{a} \in \mathbf{A}$, we substitute $\Lambda_{\mathbf{a}}=1$ from (\ref{La}), quantities as and the expression of from (4.12) into the inequality (4.7) to deduce (\ref{mainform})
Note that for every $\mathbf{a} \in \mathbf{A}$, $\Lambda_{\mathbf{a}}=1$. Thus, the interpolating polynomial is given by the following expression:
\begin{eqnarray*}
\label{tril}
        f(x_1,x_2,x_3) &=& c_{000}(1-x_1)(1-x_2)(1-x_3)+c_{001}(1-x_1)x_2(1-x_3)  \\&& +  c_{010}(1-x_1)x_2(1-x_3) 
        + c_{100}x_1(1-x_2)(1-x_3) + c_{011}(1-x_1)x_2x_3\\&& 
        + c_{101} x_1 x_2 (1-x_3) 
        +c _{110}x_1x_2(1-x_3) +c_{111}x_1x_2x_3
    \end{eqnarray*}
    
    Observe that the above expression is identical to the trilinear interpolating polynomial  for the unit step grid.
    
\end{exam}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{exam}\label{gridfun3}
{\rm

Consider the function %$\displaystyle 
$ g(x_1,x_2,x_3) =  x_1 \sin(x_2)+ \frac{x_2 \sin(x_1)}{10}-x_1 \sin\left(\frac{x_2 x_3}{4}\right)$, and the grid of support points $\mathbf{A}=A_1 \times A_2 \times A_3$, where $A_1 =A_2=A_3= \{-7,-6,\dots,7\}$, with multiplicity function $v(\mathbf{a}) = (v_1(\mathbf{a}),\;v_2(\mathbf{a}),\;v_3(\mathbf{a})) = (1,1,1) , (2,2,2)$, for every point on the grid, $\mathbf{a} \in \mathbf{A}$. Thus, in total we utilize $15 \times 15 \times 15$ support points to derive the Hermite interpolating polynomial. 

In this example we use the values of $g$ and its partial derivatives up to maximum order,  $v(\mathbf{a})-1$, at each support point $\mathbf{a}$, to interpolate the function at $57 \times 57 \times 57$ equally distributed points in $[-7,7] \times [-7,7] \times [-7,7]$. The cubic spline, linear, cubic polynomial and the Hermit Makima interpolation methods are also applied at the same points. The achieved RMSE by each method is shown in Table \ref{table4}, calculated at the aforementioned points.

In addition, we implement the Hermit interpolation via splines, where we use a smaller grid. Namely, for the current example, the grid of spline support points $\mathbf{B}=B_1 \times B_2 \times B_3$, where $B_1 =B_2=B_3= \{0,1,2\}$, with multiplicity function $v(\mathbf{b}) = (v_1(\mathbf{b}),\;v_2(\mathbf{b}),\;v_3(\mathbf{b})) = (2,2,2)$, for every point on the grid, $b \in \mathbf{B}$.

\begin{table}[!h]
\begin{center}
\caption{The achieved RMSE for the proposed Hermite polynomial and other interpolation methods, in the case of Example \ref{examp3d}}\label{table4}
\begin{tabular}{|l cc|}
\hline
Method & RMSE &\\ \hline
%Proposed Hermite $v(\mathbf{a}) = (1,1,1)$ &   & \\ \hline
Proposed Hermite $v(\mathbf{a}) = (2,2,2)$ &   0.0015 & \\ \hline
Linear & 1.3318 &  \\ \hline
Cubic   &  0.6699 &  \\ \hline
Makima  &  0.7748 & \\ \hline
Spline  &    0.7461 & \\ \hline
\hline
\end{tabular}

\end{center} 
\end{table}

\begin{figure}[!h]
     \centering
         \includegraphics[width=16cm]{fig3D_1.png}%{3d_1_250.png}
         \caption{Function $ g(x_1,x_2,x_3) =  x_1 \sin(x_2)+ \frac{x_2 \sin(x_1)}{10}-x_1 \sin\left(\frac{x_2 x_3}{4}\right)$ of Example \ref{gridfun3}}
         \label{figgr}
\end{figure}

} 
\end{exam}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
\begin{exam}\label{examp8}
{\rm
Consider the function of Example \ref{gridfun3}, $ g(x_1,x_2,x_3) =  x_1 \sin(x_2)+ \frac{x_2 \sin(x_1)}{10}-x_1 \sin\left(\frac{x_2 x_3}{4}\right)$ and the support points arranged on the same 3D grid. The task is to interpolate the values of this function at the points of a plane $\pi$, as shown in Fig(\ref{plane}). The interpolation is performed for $(x_{1},x_{2},\pi(x_{1},x_{2})$, with $(x_{1},x_{2}) \in [1,18]\times[1,18]$ and $\pi$ is the plane through point $(10.5,10.5,10.5)$ with normal vector equal to $\left(\frac{1}{\sqrt{2}},0,\frac{1}{\sqrt{2}}\right)$.  To this end, we utilize the proposed Hermite interpolation as splines $B=B_1 \times B_2 \times B_3$ 

\begin{table}[!h]
\begin{center}
\caption{The achieved RMSE for the proposed Hermite spline polynomial and other interpolation methods, in the case of Example \ref{examp8}}\label{table8}
\begin{tabular}{|l cc|}
\hline
Method & RMSE &\\ \hline
Proposed Hermite spline $3\times 3 \times 3$, $v(\mathbf{a}) = (2,2,2)$ &  1.2297 & \\ \hline
Proposed Hermite spline $3\times 3 \times 3$, $v(\mathbf{a}) = (3,3,3)$ &  0.0678  & \\ \hline
Proposed Hermite spline $5\times 5 \times 5$, $v(\mathbf{a}) = (2,2,2)$ &  0.3674  & \\ \hline
Proposed Hermite spline $5\times 5 \times 5$, $v(\mathbf{a}) = (3,3,3)$ &  0.0020  & \\ \hline
Linear & 5.5936 &  \\ \hline
Cubic   & 5.3674 &  \\ \hline
Makima  &  5.3271 & \\ \hline
Spline  &  5.6318 & \\ \hline
\hline
\end{tabular}
\end{center} 
\end{table}
\begin{comment}

\begin{figure}[!h]
     \centering
         \includegraphics[width=11cm]{plane1.png}
         \caption{Spline  interpolation along an oblique plane of function $ g(x_1,x_2,x_3) =  x_1 \sin(x_2)+ \frac{x_2 \sin(x_1)}{10}-x_1 \sin\left(\frac{x_2 x_3}{4}\right)$
         \label{plane}. Only the first $6 \times 6\times 6$ support points are displayed, for clarity.}
\end{figure}

\end{comment}

\begin{figure}[h!]
%\ContinuedFloat
\centering
\subfigure[]{{\includegraphics[width=0.5\textwidth]{plane1.png}}}\hfill
\subfigure[]{{\includegraphics[width=0.5\textwidth]{function_plane_with_colorbar.png}}}\hfill
\subfigure[]{{\includegraphics[width=0.55\textwidth]{fig_differences.png}}}
\caption{Spline  interpolation along an oblique plane of function $ g(x_1,x_2,x_3) =  x_1 \sin(x_2)+ \frac{x_2 \sin(x_1)}{10}-x_1 \sin\left(\frac{x_2 x_3}{4}\right)$
(a)  the first $6 \times 6\times 6$ support points are displayed, for clarity, with the oblique plane superimposed (b) the actual values of function $g$ along the oblique plane and (c) the interpolation error (difference from the actual function values) achieved by the proposed Hermite interpolation for multiplicity $\nu (\mathbf{a})=(2,2,2)$ and $\nu(\mathbf{a})=(3,3,3)$, as well as the other methods.}
\label{plane}
\end{figure}



}
\end{exam}

==> idealconn.tex <==
Let us consider the polynomials $f_{i}\in \Bbbk \left[ x_{i}\right], ~i=1,\dots,n,$  $A_{i}$ the sets of their roots in the algebraic closure $\overline{\Bbbk }$
of $\Bbbk $, and $\nu _{i}\left( a\right) $ the multiplicity of $a\in A_{i}$. 
Therefore $f_{i}\left( x_{i}\right) =\prod_{a\in A_{i}}\left( x_{i}-a\right)
^{\nu _{i}\left( a\right) },~i=1,\dots,n$. 
Furthermore, we denote by $I$ the ideal of $\Bbbk \left[ x_{1},\dots,x_{n}\right] $
generated by $f_{1},\dots,f_{n}$, and by $\overline{I}$ the ideal of $%
\overline{\Bbbk }\left[ x_{1},\dots,x_{n}\right] $ generated by $%
f_{1},\dots,f_{n}$. 
 For $g\in \Bbbk \left[ x_{1},\dots,x_{n}\right] $ let us denote by\ $
\widetilde{g}$ the residue class of $g$ in $\Bbbk \left[ x_{1},\dots,x_{n}%
\right] /I$ , and by $\overline{g}\ $the residue class of $g$\ in $\overline{%
\Bbbk }\left[ x_{1},\dots,x_{n}\right] /\overline{I}$ and $J\left( \mathbf{A,}\nu \right) :=\left\{ f\in \overline{\Bbbk }\left[
x_{1},\dots,x_{n}\right] :\,\partial _{\mathbf{a}}^{\mathbf{m}}f=0,~\mathbf{%
a\in A},\; \mathbf{m\in }\left[ \mathbf{0,}\nu \left( \mathbf{a}\right) -%
\mathbf{1}\right] \right\} $. Similarly to Remark \ref{rem8} it can be shown that $
J\left( \mathbf{A,}\nu \right) $ is an ideal of $\overline{\Bbbk }\left[
x_{1},\dots,x_{n}\right] .$

\begin{lem}\label{lem41}
The $\overline{\Bbbk }$-algebra $\overline{\Bbbk }\left[ x_{1},\dots,x_{n}%
\right] /J\left( \mathbf{A,}\nu \right) $ as a $\overline{\Bbbk }-$vector
space is isomorphic to $V\left( \mathbf{A,}\nu \right) $, and 
\begin{equation*}
\dim _{\overline{\Bbbk }}\overline{\Bbbk }\left[ x_{1},\dots,x_{n}\right]
/J\left( \mathbf{A,}\nu \right) =\prod_{i=1}^{n}\sum_{a_{i}\in A_{i}}\nu
_{i}\left( a\right).
\end{equation*}
\end{lem}

\begin{proof}
Let $\phi :\overline{\Bbbk }\left[ x_{1},\dots,x_{n}\right] \rightarrow 
\overline{\Bbbk }\left[ x_{1},\dots,x_{n}\right] /J\left( \mathbf{A,}\nu
\right) $ be the canonical map and $B\left( \mathbf{A,}\nu \right) :=\left\{ \mathbf{x}^{%
\mathbf{k}}:\mathbf{k\in }\left[ \mathbf{0,}-\mathbf{1+}\sum_{\mathbf{a\in A}%
}\nu \left( \mathbf{a}\right) \right] \right\}$ a basis of the vector space $V\left( \mathbf{A,}%
\nu \right) $. It is sufficient to show
that $\phi \left( B\left( \mathbf{A,}\nu \right) \right) $ is a basis of $K%
\left[ x_{1},\dots,x_{n}\right] /J\left( \mathbf{A,}\nu \right)$. Starting
from $\sum_{\mathbf{k\in }\left[ \mathbf{0,}-\mathbf{1+}\sum_{\mathbf{a\in A}%
}\nu \left( \mathbf{a}\right) \right] }c_{\mathbf{k}}\phi \left( \mathbf{x}^{%
\mathbf{k}}\right) =0$, we have $\sum_{\mathbf{k\in }\left[ \mathbf{0,}-%
\mathbf{1+}\sum_{\mathbf{a\in A}}\nu \left( \mathbf{a}\right) \right] }c_{%
\mathbf{k}}$\textbf{$x$}$^{\mathbf{k}}\in J\left( \mathbf{A,}\nu \right) $,
or equivalently $\partial _{\mathbf{a}}^{\mathbf{m}}\sum_{\mathbf{k\in }%
\left[ \mathbf{0,}-\mathbf{1+}\sum_{\mathbf{a\in A}}\nu \left( \mathbf{a}%
\right) \right] }c_{\mathbf{k}}$\textbf{$x$}$^{\mathbf{k}}=0$, so according
to Corollary \ref{cor24} $\sum_{\mathbf{k\in }\left[ \mathbf{0,}-\mathbf{1+}%
\sum_{\mathbf{a\in A}}\nu \left( \mathbf{a}\right) \right] }c_{\mathbf{k}}$%
\textbf{$x$}$^{\mathbf{k}}=0$. That is $c_{\mathbf{k}}=0$, $\mathbf{k\in }%
\left[ \mathbf{0,}-\mathbf{1+}\sum_{\mathbf{a\in A}}\nu \left( \mathbf{a}%
\right) \right]$, which means that $\phi \left( \mathbf{x}^{\mathbf{k}}\right),
\mathbf{k\in }\left[ \mathbf{0,}-\mathbf{1+}\sum_{\mathbf{a\in A}}\nu \left( 
\mathbf{a}\right) \right] $ are linearly indepedend. Now we will show that $%
\phi \left( \mathbf{x}^{\mathbf{k}}\right) ,\mathbf{k\in }\left[ \mathbf{0,}-%
\mathbf{1+}\sum_{\mathbf{a\in A}}\nu \left( \mathbf{a}\right) \right] $
generate $\Bbbk \left[ x_{1},\dots,x_{n}\right] /J\left( \mathbf{A,}\nu
\right) $: By Theorem \ref{thm1}, for any $g\in \Bbbk \left[ x_{1},\dots,x_{n}\right] 
$ there is exactly one $f=\sum_{\mathbf{k\in }\left[ \mathbf{0,}-\mathbf{1+}%
\sum_{\mathbf{a\in A}}\nu \left( \mathbf{a}\right) \right] }c_{\mathbf{k}}$%
\textbf{$x$}$^{\mathbf{k}}\in V\left( \mathbf{A,}\nu \right) $ such that $%
\partial _{\mathbf{a}}^{\mathbf{m}}f=\partial _{\mathbf{a}}^{\mathbf{m}}g,$ $%
\mathbf{a\in A},~\mathbf{m\in }\left[ \mathbf{0,}\nu \left( \mathbf{a}%
\right) -\mathbf{1}\right]$. Consequently, $\phi \left( g\right) =\phi
\left( f\right) $ or 
\begin{equation*}
\phi \left( g\right) =\sum_{\mathbf{k\in }\left[ \mathbf{0,}-\mathbf{1+}%
\sum_{\mathbf{a\in A}}\nu \left( \mathbf{a}\right) \right] }c_{\mathbf{k}%
}\phi \left( \mathbf{x}^{\mathbf{k}}\right) .
\end{equation*}
\end{proof}

\begin{lem}
%If $\left( f_{1},\dots,f_{n}\right) $ is the ideal of $\Bbbk \left[x_{1},\dots,x_{n}\right] $ generated by the polynomials $f_{1}\in \Bbbk \left[x_{1}\right] ,\dots,f_{n}\in \Bbbk \left[ x_{n}\right] $, then 
The quotient
ring $\Bbbk \left[ x_{1},\dots,x_{n}\right] /I$ as a $\Bbbk$-vector space is
isomorphic to $V\left( \mathbf{A,}\nu \right) $, and  
\begin{equation*}
\dim _{\Bbbk }\Bbbk \left[ x_{1},\dots,x_{n}\right] /I=\prod_{i=1}^{n}\deg
f_{i}=\prod_{i=1}^{n}\sum_{a_{i}\in A_{i}}\nu _{i}\left( a\right) .
\end{equation*}
\end{lem}

\begin{proof}
Clearly, it is sufficient to prove that for any polynomial $f\in \Bbbk \left[ x_{1},\dots,x_{n}%
\right] $ there exist unique $c_{\left( k_{1},\dots,k_{n}\right) }\in K,~0\leq
k_{1}<\deg f_{1},\dots,0\leq k_{n}<\deg f_{n}$, such that 
\begin{equation*}
f=\sum_{k_{1}=0}^{\deg f_{1}-1}\dots\sum_{k_{n}=0}^{\deg f_{n}-1}c_{\left(
k_{1},\dots,k_{n}\right) }x_{1}^{k_{1}}\dots x_{n}^{k_{n}}+I.
\end{equation*}%
To this end we will apply the method of induction over $n$. For $n=1$ obviously the claim is valid. Let the claim be valid for $n-1,n>1$%
. From $f\in \Bbbk \left[ x_{1},\dots,x_{n-1}\right] \left[ x_{n}\right] $, by
dividing $f$ $\ $by $f_{n}\left( x_{n}\right) $, we have $f=pf_{n}+q,$ where 
$p,q\in \Bbbk \left[ x_{1},\dots,x_{n}\right] $ are uniquely determined
by $\deg _{n}q<\deg f_{n}$. Therefore 
\begin{equation}\label{taged31}
f=\sum_{i=0}^{-\deg f_{n}-1}q_{i}x_{n}^{i}+\left( f_{n}\right), 
\end{equation}%
where $q_{i}$ are uniquely determined polynomials of $\Bbbk \left[
x_{1},\dots,x_{n-1}\right] $, and $\left( f_{n}\right) $ is the ideal of $%
\Bbbk \left[ x_{1},\dots,x_{n}\right] $ generated by $f_{n}$. Now by induction
the polynomials $q_{i}$ can be written as, 
\begin{equation}\label{taged32}
q_{i}=\sum_{0\leq k_{1}<\deg f_{1}}\dots \sum_{0\leq k_{n-1}<\deg
f_{n-1}}c_{\left( k_{1},\dots,k_{n-1}\right)
}^{i}x_{1}^{k_{1}}\dots x_{n-1}^{k_{n-1}}+\left( f_{1},\dots,f_{n-1}\right) , 
\end{equation}%
where $c_{\left( k_{1},\dots,k_{n-1}\right) }^{i}\in \Bbbk $ are uniquely
determined$.$ Putting (\ref{taged32}) in (\ref{taged31}) we obtain the claim.
\end{proof}

\begin{thm}\label{them43}
The following holds  
$$\overline{I}=J\left( \mathbf{A,}\nu \right) $$
\end{thm}

\begin{proof}
We can write $f_{i}$ as, $f_{i}\left( x_{i}\right) =\prod_{a\in
A_{i}}\left( x_{i}-a\right) ^{\nu _{i}\left( a\right) },~i=1,\dots,n.$ By
Leibniz derivative rule we easily conclude that for each $g\in \overline{%
\Bbbk }\left[ x_{1},\dots,x_{n}\right] $ is valid $\partial _{\mathbf{a}}^{%
\mathbf{m}}\left( gf_{\iota }\right) =0$, for each $\mathbf{a\in A},~\mathbf{%
m\in }\left[ \mathbf{0,}\nu \left( \mathbf{a}\right) -\mathbf{1}\right] .$
Therefore $f_{i}\in J\left( \mathbf{A,}\nu \right) ,~i=1,\dots,n.$ That is 
\begin{equation}\label{taged33}
\overline{I}\subseteq J\left( \mathbf{A,}\nu \right) .
\end{equation}%
It is sufficient \ to show $J\left( \mathbf{A,}\nu \right) \subseteq 
\overline{I}$: Let $g$ be any element of $\overline{I}$. By Lemma \ref{lem41} there
is unique polynomial $p\in V\left( \mathbf{A,}\nu \right) $ such that 
\begin{equation} \label{taged34}
g=p+\overline{I}  
\end{equation}%
From (\ref{taged34}) we have that for any $\mathbf{m\in }\left[ \mathbf{%
0,}\nu \left( \mathbf{a}\right) -\mathbf{1}\right] $ and any$~\mathbf{a\in A}
$ 
\begin{equation*}
\partial _{\mathbf{a}}^{\mathbf{m}}g=\partial _{\mathbf{a}}^{\mathbf{m}}p,
\end{equation*}%
which implies $\partial _{\mathbf{a}}^{\mathbf{m}}p=0$. Therefore by
Corollary 2.4 \ is valid $p=0,$ which combined with (\ref{taged34})
gives $g\in \overline{I}.$
\end{proof}

\begin{cor}
The following holds $$I=J\left( \mathbf{A,}\nu \right) \cap \Bbbk \left[ x_{1},\dots,x_{n}\right].$$
%that is $f\in I$ if and only if $\ \partial _{\mathbf{a}}^{\mathbf{m}}f=0$
%for each $\mathbf{a\in A}$ and$~\mathbf{m\in }\left[ \mathbf{0,}\nu \left( \mathbf{a}\right) -\mathbf{1}\right] .$
\end{cor}

\begin{proof}
By Theorem \ref{them43} we immediately get $I\subseteq J\left( \mathbf{A,}\nu \right)
\cap \Bbbk \left[ x_{1},\dots,x_{n}\right] $. Therefore it is sufficient to
prove $J\left( \mathbf{A,}\nu \right) \cap \Bbbk \left[ x_{1},\dots,x_{n}%
\right] \subseteq I:$ \ Let $f$ be any element of $J\left( \mathbf{A,}\nu
\right) \cap \Bbbk \left[ x_{1},\dots,x_{n}\right] .$ Then by Theorem \ref{them43} we have%
\begin{equation}\label{taged36}
f=\sum_{i=1}^{n}f_{i}g_{i},
\end{equation}%
where $g_{i}\in \overline{\Bbbk }\left[ x_{1},\dots,x_{n}\right] .$ Consider
the finite field extension $\Bbbk \subset \Bbbk _{1}$, where $\Bbbk _{1}$ is
the field constructed by adjunction of all coefficients of the polynomials $%
g_{i}.$ Let $r$ be the degree of $\Bbbk \subset \Bbbk _{1}$ and $\rho $ a
primitive element. Then (\ref{taged36}) can be written as 
\begin{equation}\label{taged37}
f=\sum_{j=0}^{r-1}\rho ^{j}\sum_{i=1}^{n}f_{i}g_{ij},  
\end{equation}%
where $g_{ij}\in \Bbbk \left[ x_{1},\dots,x_{n}\right] .$ Finally, since $%
\left\{ 1,\rho ,\dots,\rho ^{n-1}\right\} $ is $\Bbbk -$ linearly indepedent,
one from (\ref{taged37}) has
\begin{equation*}
f=\sum_{i=1}^{n}f_{i}g_{ij}.
\end{equation*}
\end{proof}
In other words $f\in I$, if and only if $I=J\left( \mathbf{A,}\nu \right) \cap \Bbbk \left[ x_{1},\dots,x_{n}\right]$.


==> imagesupreds.tex <==
%%%%%%%%%%%%%%%

\begin{comment}


\begin{table}[!h]
\begin{center}
\caption{The achieved RMSE for the proposed Hermite spline polynomial and other interpolation methods, in the case of Example \ref{}}\label{tably1}
\begin{tabular}{|l |ccc|}
\hline
\textbf{Method} &  \multicolumn{3}{c|}{\textbf{Scale Factor}} \\ 
& $\times 2$ & $\times 3$ & $\times 4$\\ \hline
Hermite $5\times 5 $, $v(\mathbf{a}) = (3,3)$ &  & &  \\ \hline
Hermite $5\times 5 \times 5$, $v(\mathbf{a}) = (2,2)$ &  &  &  \\ \hline
Hermite $3\times 3 $, $v(\mathbf{a}) = (3,3)$   &  & & \\ \hline
Hermite $3\times 3 $, $v(\mathbf{a}) = (2,2)$ &   &  &   \\ \hline
OMOMS $\deg 4$ & & & \\ \hline
OMOMS $\deg 7$ &  &  & \\ \hline
B-spline $\deg 7$ &  & &  \\ \hline
EDSR   & & &  \\ \hline
ESPCN & & & \\ \hline
FSRCNN &  & & \\ \hline
LapSRN &  & &  \\ \hline
Makima  &   &  & \\ \hline
\end{tabular}

\end{center} 
\end{table}

    
\end{comment}

==> newdef.tex <==
In this section we provide a quick proof of Theorem \ref{th1}, as an alternative to the proof given in \cite{fractmult}. 
In addition to the already defined $H_{a}^{k}(x)$, we define the following

%    \item Let $A$ be a finite subset of $\Bbbk $. Then for any $a\in A$ and $%    k\in \left\{ 1,\dots,\nu \left( a\right) -1\right\} $,     \begin{equation*}    H_{a}^{k}\left( x\right) :=H_{a}\left( x\right) \frac{\left( x-a\right) ^{k}%    }{k!}\sum_{t=0}^{\nu \left( a\right) -k-1}\frac{\left( x-a\right) ^{t}}{t!}    \left( \frac{1}{H_{a}\left( x\right) }\right) ^{\left( t\right) }\left(    a\right) \in \Bbbk \left[ x\right] ,    \end{equation*} where the superscript $(t)$ indicates order of derivative.


\begin{equation*}
H_{\mathbf{a}}^{\mathbf{k}}\left( x_{1},\dots, x_{n}\right)
:=\prod_{i=1}^{n}H_{a_{i}}^{k_{i}}\left( x_{i}\right) \in \Bbbk \left[
x_{1},\dots,x_{n}\right], \text{ and}
\end{equation*}

%Let us define $Q\left( \mathbf{A,}\nu \right)$ as follows

\begin{equation*}
Q\left( \mathbf{A,}\nu \right) :=\left\{ H_{\mathbf{a}}^{\mathbf{k}}:\mathbf{%
a\in A}\text{, }\mathbf{k\in }\left[ \mathbf{0,}\nu \left( \mathbf{a}\right)
-\mathbf{1}\right] \right\} .
\end{equation*}

First, we state the following remarks and lemma.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
\begin{rem}\label{rem9}
{\rm
From $\deg _{i}H_{\mathbf{a}}^{\mathbf{k}}=k_{i}+\sum_{a\in A_{i}-\left\{
a_{i}\right\} }\nu _{i}\left( a\right) <\sum_{a\in A_{i}}\nu _{i}\left(
a\right) $ follows $Q\left( \mathbf{A,}\nu \right) \subset V\left( \mathbf{A,%
}\nu \right) $, and $\left\vert Q\left( \mathbf{A,}\nu \right) \right\vert
=\prod_{i=1}^{n}\sum_{a_{i}\in A_{i}}\nu _{i}\left( a\right) =\dim
_{k}V\left( \mathbf{A,}\nu \right) .$}
\end{rem}

\begin{rem}\label{remkron}
{\rm
For any $a,~b\in A$, and $k,m\in \left\{ 1,\dots,\nu \left( a\right)
-1\right\} $ we have (see \cite{SPITZ})
\begin{equation*}
\partial ^{m}H_{a}^{k}\left( b\right) =\left\{ 
\begin{array}{ccc}
0, & \text{if} & a\neq b \\ 
\delta _{km} & \text{if} & a=b%
\end{array}%
\right. ,
\end{equation*}%
where $\delta _{km}$ is the Kronecker Delta. From this we immediately
obtain, for any $\mathbf{a,b\in A}$, and any $~\mathbf{k,~m\in }\left[ 
\mathbf{0,}\nu \left( \mathbf{a}\right) -\mathbf{1}\right] $ we have%
\begin{equation*}
\partial _{\mathbf{a}}^{\mathbf{m}}H^{\mathbf{k}}\left( \mathbf{b}\right)
=\left\{ 
\begin{array}{ccc}
0, & \text{if} & \mathbf{a}\neq \mathbf{b} \\ 
\delta _{\mathbf{km}} & \text{if} & \mathbf{a}=\mathbf{b}%
\end{array}%
\right. .
\end{equation*}}
\end{rem}

\begin{lem}\label{lemex}
$Q\left( \mathbf{A,}\nu \right) $ is a basis of $V\left( \mathbf{A,}\nu
\right)$.
\end{lem}

\begin{proof}
By Remark \ref{rem9} it is sufficient to show that $Q\left( \mathbf{A,}\nu
\right) $ is linearly independent: From $\sum_{\mathbf{b\in A}}\sum_{\mathbf{%
k\in }\left[ \mathbf{0,}\nu \left( \mathbf{b}\right) -\mathbf{1}\right] }c_{%
\mathbf{b}}^{\mathbf{m}}H_{\mathbf{b}}^{\mathbf{m}}=0,~c_{\mathbf{b}}^{%
\mathbf{m}}\in 
%TCIMACRO{\U{2102} }%
%BeginExpansion
\mathbb{C}
%EndExpansion
$ for each $\mathbf{a\in A,~k\in }\left[ \mathbf{0,}\nu \left( \mathbf{a}%
\right) -\mathbf{1}\right] $ follows $\sum_{\mathbf{b\in A}}\sum_{\mathbf{%
k\in }\left[ \mathbf{0,}\nu \left( \mathbf{b}\right) -\mathbf{1}\right] }c_{%
\mathbf{b}}^{\mathbf{m}}\partial _{\mathbf{a}}^{\mathbf{k}}H_{\mathbf{b}}^{%
\mathbf{m}}=0,$ from which by Remark \ref{remkron} we conclude $c_{\mathbf{a}}^{%
\mathbf{k}}=0$.
\end{proof}




\begin{thm}
Given $t_{\mathbf{a}}^{\mathbf{k}}\in \,,~\mathbf{a\in A},~\mathbf{k\in }%
\left[ \mathbf{0,}\nu \left( \mathbf{a}\right) -\mathbf{1}\right] .$ Then
there is a unique $p\in V\left( \mathbf{A,}\nu \right) $ such that $\partial
_{\mathbf{a}}^{\mathbf{k}}p=t_{\mathbf{a}}^{\mathbf{k}},~\mathbf{a\in A}, $ $
\mathbf{k\in }\left[ \mathbf{0,}\nu \left( \mathbf{a}\right) -\mathbf{1}%
\right] $, and $p$ is given by 
\begin{equation*}
p=\sum_{\mathbf{a\in A}}\sum_{\mathbf{m\in }\left[ \mathbf{0,}\nu \left( 
\mathbf{a}\right) -\mathbf{1}\right] }t_{\mathbf{a}}^{\mathbf{k}}H_{\mathbf{a%
}}^{\mathbf{k}}=\sum_{a_{1}\in A_{1}}\dots\sum_{a_{n}\in
A_{n}}\sum_{k_{n}=0}^{\nu _{1}\left( a_{1}\right) -1}\dots\sum_{k_{n}=0}^{\nu
_{n}\left( a_{n}\right) -1}\ \prod_{j=1}^{n}\partial
_{i}^{k}H_{a_{j}}^{k_{j}}\left( x_{j}\right) t_{\mathbf{a}}^{\mathbf{k}}.
\end{equation*}
\end{thm}

\begin{proof}
By Remark \ref{remkron} for each $\mathbf{a\in A,~k\in }\left[ \mathbf{0,}\nu \left( 
\mathbf{a}\right) -\mathbf{1}\right] $ we have 
\begin{equation*}
\partial _{\mathbf{a}}^{\mathbf{k}}p=\sum_{\mathbf{b\in A}}\sum_{\mathbf{%
k\in }\left[ \mathbf{0,}\nu \left( \mathbf{b}\right) -\mathbf{1}\right] }t_{%
\mathbf{b}}^{\mathbf{m}}\partial _{\mathbf{a}}^{\mathbf{k}}H_{\mathbf{b}}^{%
\mathbf{m}}=t_{\mathbf{a}}^{\mathbf{k}}.
\end{equation*}
The uniqueness of $p$ follows\ By Lemma \ref{lemex}.
\end{proof}

==> onideal_new.tex <==
Let $A_{i},\;i=1,\dots,n,$ be finite subsets of an infinite field $\Bbbk $, and $\nu _{i}\left( a\right) $ the multiplicity of $a\in A_{i}$. Consider the polynomials $$
H_{i}\left( x_{i}\right) =\prod_{a\in A_{i}}\left(
x_{i}-a\right) ^{\nu _{i}\left( a\right) }\in \Bbbk \left[ x_{i}\right]
,\;i=1,\dots,n.$$

For $g\in \Bbbk \left[ x_{1},\dots,x_{n}\right] $, denote by\ $
\widetilde{g}$ the residue class of $g$ in the quotient ring $\Bbbk \left[
x_{1},\dots,x_{n}\right] /\left( H_{1},\dots,H_{n}\right) $. It is easy to verify that the linear operator $T_{\left( \mathbf{A,}\nu
,\Bbbk \right) }:\Bbbk \left[ x_{1},\dots,x_{n}\right] \rightarrow $ $V\left( 
\mathbf{A,}\nu \right) $, given by 
\begin{equation*}
T_{\left( \mathbf{A,}\nu ,\Bbbk \right) }\left( f\right) =\sum_{\mathbf{a\in
A}}\sum_{\mathbf{k\in }\left[ \mathbf{0,}\nu \left( \mathbf{a}\right) -%
\mathbf{1}\right] }H_{\mathbf{a}}^{\mathbf{k}}\partial _{\mathbf{a}}^{%
\mathbf{k}}f,
\end{equation*}%
is a projector. Further, similarly to Remark $8,$ it can be shown that $\ker
T_{\left( \mathbf{A,}\nu ,\Bbbk \right) }$ is an ideal of $\Bbbk \left[
x_{1},\dots,x_{n}\right] $. So $T_{\left( \mathbf{A,}\nu ,\Bbbk \right) }$ is
an ideal projector.

\begin{lem}
The $\Bbbk$-algebra $\Bbbk \left[ x_{1},\dots,x_{n}\right] /\ker T_{\left( 
\mathbf{A,}\nu ,\Bbbk \right) }$ as a $\Bbbk$-vector space is isomorphic to 
$V\left( \mathbf{A,}\nu \right) $, and the following is valid 
\begin{equation*}
\dim _{\Bbbk }\Bbbk \left[ x_{1},\dots,x_{n}\right] /\ker T_{\left( \mathbf{A,}%
\nu ,\Bbbk \right) }=\prod_{i=1}^{n}\sum_{a_{i}\in A_{i}}\nu _{i}\left(
a\right)
\end{equation*}
\end{lem}
\begin{proof}
Let $\phi :\Bbbk \left[ x_{1},\dots,x_{n}\right] \rightarrow \Bbbk \left[
x_{1},\dots,x_{n}\right] /\ker T_{\left( \mathbf{A,}\nu ,\Bbbk \right) }$be
the canonical map. Consider any basis $B$ of the vector space $V\left( 
\mathbf{A,}\nu \right) .$ It is sufficient to show, that $\phi \left(
B\right) $ is a basis of $\Bbbk \left[ x_{1},\dots,x_{n}\right] /\ker
T_{\left( \mathbf{A,}\nu ,\Bbbk \right) }:$ Starting from $\sum_{b\mathbf{%
\in }B}c_{b}\phi \left( b\right) =0$, $c_{b}\in \Bbbk $ we have $\sum_{b%
\mathbf{\in }B}c_{b}\phi \left( b\right) \in \ker T_{\left( \mathbf{A,}\nu
,\Bbbk \right) }$, from which we obtain 
\begin{equation*}
\partial _{\mathbf{a}}^{\mathbf{m}}\sum_{b\mathbf{\in }B}c_{b}b=0,~\mathbf{%
a\in A}\text{ and}~\mathbf{m\in }\left[ \mathbf{0,}\nu \left( \mathbf{a}%
\right) -\mathbf{1}\right] .
\end{equation*}%
Further $~$because $B\subset V\left( \mathbf{A,}\nu \right) $ we have$\
\sum_{b\mathbf{\in }B}c_{b}b\in V\left( \mathbf{A,}\nu \right) .$%
Consequently by Corollary 2.4 holds $\sum_{b\mathbf{\in }B}c_{b}b=0.~$%
Terefore for each $b\mathbf{\in }B$ holds $c_{b}=0,$which means $\phi \left(
B\right) $ is linearly indepedend. Now we will show that $\phi \left(
B\right) $ generate $\Bbbk \left[ x_{1},\dots,x_{n}\right] /\ker T_{\left( 
\mathbf{A,}\nu ,\Bbbk \right) }$: By Theorem 2.2, for any $g\in \Bbbk \left[
x_{1},\dots,x_{n}\right] $ there is exact one $f=\sum_{b\mathbf{\in }%
B}c_{b}b\in V\left( \mathbf{A,}\nu \right) $ such that $\partial _{\mathbf{a}%
}^{\mathbf{m}}f=\partial _{\mathbf{a}}^{\mathbf{m}}g,$ $\mathbf{a\in A},~%
\mathbf{m\in }\left[ \mathbf{0,}\nu \left( \mathbf{a}\right) -\mathbf{1}%
\right] .$ Consequently $\phi \left( g\right) =\phi \left( f\right) $, which
can be written as 
\begin{equation*}
\phi \left( g\right) =\sum_{b\mathbf{\in }B}c_{b}\phi \left( b\right) .
\end{equation*}
\end{proof}

\begin{comment}

\begin{proof}
Let $\phi :\Bbbk \left[ x_{1},\dots,x_{n}\right] \rightarrow \Bbbk \left[
x_{1},\dots,x_{n}\right] /\ker T_{\left( \mathbf{A,}\nu ,\Bbbk \right) }$ be
the canonical map. We will use the basis $B\left( \mathbf{A,}\nu \right) :=\left\{ \mathbf{x}^{\mathbf{k}%
}:\mathbf{k\in }\left[ \mathbf{0,}-\mathbf{1+}\sum_{\mathbf{a\in A}}\nu
\left( \mathbf{a}\right) \right] \right\}$ of the vector space $V\left( \mathbf{A,}\nu
\right) $. It is sufficient to show that $%
\phi \left( B\left( \mathbf{A,}\nu \right) \right) $ is a basis of $\Bbbk %
\left[ x_{1},\dots,x_{n}\right] /\ker T_{\left( \mathbf{A,}\nu ,\Bbbk \right)
}:$ Starting from $\sum_{\mathbf{k\in }\left[ \mathbf{0,}-\mathbf{1+}\sum_{%
\mathbf{a\in A}}\nu \left( \mathbf{a}\right) \right] }c_{\mathbf{k}}\phi
\left( \mathbf{x}^{\mathbf{k}}\right) =0$, we have $\sum_{\mathbf{k\in }%
\left[ \mathbf{0,}-\mathbf{1+}\sum_{\mathbf{a\in A}}\nu \left( \mathbf{a}%
\right) \right] }c_{\mathbf{k}}$\textbf{$x$}$^{\mathbf{k}}\in \ker T_{\left( 
\mathbf{A,}\nu ,\Bbbk \right) }$, or equivalently $$\partial _{\mathbf{a}}^{%
\mathbf{m}}\sum_{\mathbf{k\in }\left[ \mathbf{0,}-\mathbf{1+}\sum_{\mathbf{%
a\in A}}\nu \left( \mathbf{a}\right) \right] }c_{\mathbf{k}}\mathbf{x}^{
\mathbf{k}}=0, ~\mathbf{a\in A},~\mathbf{m\in }\left[ \mathbf{0,}\nu \left( \mathbf{a}%
\right) -\mathbf{1}\right].$$ 

Because, $\sum_{\mathbf{k\in }\left[ \mathbf{0,}-\mathbf{1+}\sum_{\mathbf{a\in A}}\nu \left( \mathbf{a}\right) \right] }c_{\mathbf{k}}\mathbf{x}^{
\mathbf{k}}\in  V\left( \mathbf{A,}\nu
\right)$ and according to Corollary \ref{cor24}, it follows $\sum_{\mathbf{k\in }%
\left[ \mathbf{0,}-\mathbf{1+}\sum_{\mathbf{a\in A}}\nu \left( \mathbf{a}%
\right) \right] }c_{\mathbf{k}}$\textbf{$x$}$^{\mathbf{k}}=0$, which yields $c_{
\mathbf{k}}=0$, $\mathbf{k\in }\left[ \mathbf{0,}-\mathbf{1+}\sum_{\mathbf{%
a\in A}}\nu \left( \mathbf{a}\right) \right] .$That means $\phi \left( 
\mathbf{x}^{\mathbf{k}}\right) ,\mathbf{k\in }\left[ \mathbf{0,}-\mathbf{1+}
\sum_{\mathbf{a\in A}}\nu \left( \mathbf{a}\right) \right] $ are linearly
indepedend. Now we will show that $\phi \left( \mathbf{x}^{\mathbf{k}%
}\right) ,\mathbf{k\in }\left[ \mathbf{0,}-\mathbf{1+}\sum_{\mathbf{a\in A}%
}\nu \left( \mathbf{a}\right) \right] $ generate $\Bbbk \left[
x_{1},\dots,x_{n}\right] /\ker T_{\left( \mathbf{A,}\nu ,\Bbbk \right) }$: By
Theorem 2.2, for any $g\in \Bbbk \left[ x_{1},\dots,x_{n}\right] $ there is
exactly one $$f=\sum_{\mathbf{k\in }\left[ \mathbf{0,}-\mathbf{1+}\sum_{\mathbf{%
a\in A}}\nu \left( \mathbf{a}\right) \right] }c_{\mathbf{k}}\mathbf{x}^{
\mathbf{k}}\in V\left( \mathbf{A,}\nu \right),$$ 
such that $\partial_{%
\mathbf{a}}^{\mathbf{m}}f=\partial _{\mathbf{a}}^{\mathbf{m}}g,$ $\mathbf{%
a\in A},~\mathbf{m\in }\left[ \mathbf{0,}\nu \left( \mathbf{a}\right) -%
\mathbf{1}\right]$. Consequently,  $\phi \left( g\right) =\phi \left(
f\right) $ or equivalently
\begin{equation*}
\phi \left( g\right) =\sum_{\mathbf{k\in }\left[ \mathbf{0,}-\mathbf{1+}%
\sum_{\mathbf{a\in A}}\nu \left( \mathbf{a}\right) \right] }c_{\mathbf{k}%
}\phi \left( \mathbf{x}^{\mathbf{k}}\right) .
\end{equation*}
\end{proof}
\end{comment}
\begin{lem}\label{lem42}
Given the polynomials $f_{i}\in \Bbbk \left[ x_{i}\right] ,~i=1,\dots,n~$, 
the quotient ring $\Bbbk \left[ x_{1},,x_{n}\right] /\left(
f_{1},\dots,f_{n}\right) $ as a $\Bbbk$-vector space is isomorphic to $%
\left\{ f\in 
%TCIMACRO{\U{2102} }%
%BeginExpansion
\mathbb{C}
%EndExpansion
\left[ x_{1},\dots,x_{n}\right] :\deg _{i}f<\deg f_{i},i=1,\dots,n\right\} ,$
and 
\begin{equation*}
\dim _{\Bbbk }\Bbbk \left[ x_{1},\dots,x_{n}\right] /\left(
f_{1},\dots,f_{n}\right) =\prod_{i=1}^{n}\deg f_{i}.
\end{equation*}
\end{lem}

\begin{proof}
It is sufficient to prove that for any polynomiall $f\in \Bbbk %
\left[ x_{1},\dots,x_{n}\right] $ there exist unique $c_{\left(
k_{1},\dots ,k_{n}\right) }\in \Bbbk ,~0\leq k_{1}<\deg f_{1},\dots ,0\leq
k_{n}<\deg f_{n}$, such that 
\begin{equation*}
f=\sum_{k_{1}=0}^{\deg f_{1}-1}\dots\sum_{k_{n}=0}^{\deg f_{n}-1}c_{\left(
k_{1},\dots ,k_{n}\right) }x_{1}^{k_{1}}\dots x_{n}^{k_{n}}+\left(
f_{1},\dots,f_{n}\right) .
\end{equation*}
To this end, we will apply the method of induction over $n$: For $n=1$
obviously the claim is valid. Let the claim be valid for $n-1,n>1$. Dividing $f$ $\ $by $f_{n}\left( x_{n}\right) $, we have $f=pf_{n}+q,$ where 
$p,q\in \Bbbk \left[ x_{1},\dots,x_{n}\right] $ are uniquely deteminated
holding $\deg _{n}q<\deg f_{n}$. Therefore
\begin{equation}\label{41}
f=\sum_{i=0}^{\deg f_{n}-1}q_{i}x_{n}^{i}+\left( f_{n}\right) , 
\end{equation}%
where $q_{i}$ are uniquely deteminated polynomials of $\Bbbk \left[
x_{1},\dots,x_{n-1}\right] $, and $\left( f_{n}\right) $ is the ideal of $%
\Bbbk \left[ x_{1},\dots,x_{n}\right] $ generated by $f_{n}$. Now by induction,
the polynomials $q_{i}$ can be written as, 
\begin{equation}\label{42}
q_{i}=\sum_{0\leq k_{1}<\deg f_{1}}\dots\sum_{0\leq k_{n-1}<\deg
f_{n-1}}c_{\left( k_{1},\dots,k_{n-1}\right)
}^{i}x_{1}^{k_{1}}\dots x_{n-1}^{k_{n-1}}+\left( f_{1},\dots,f_{n-1}\right) , 
\end{equation}%
where $c_{\left( k_{1},\dots,k_{n-1}\right) }^{i}\in \Bbbk $ are uniquely determined. By substitution of (\ref{42}) in (\ref{41}) we obtain the required expression.
\end{proof}

\begin{thm}\label{thm43}
The following holds $$\left( H_{1},\dots,H_{n}\right) =\ker T_{\left( \mathbf{A,}\nu
,\Bbbk \right) }.$$
\end{thm}

\begin{proof}
Applying the Leibniz derivative rule we conclude that for each $g\in \Bbbk \left[
x_{1},\dots,x_{n}\right] $ the following is valid $\partial _{\mathbf{a}}^{\mathbf{m}}\left(
gH_{\iota }\right) =0,~i=1,\dots,n\,\ $, for each $\mathbf{a\in A},~\mathbf{%
m\in }\left[ \mathbf{0,}\nu \left( \mathbf{a}\right) -\mathbf{1}\right] .$
Therefore $H_{i}\in \ker T_{\left( \mathbf{A,}\nu ,\Bbbk \right)
},~i=1,\dots,n$, or equivalently 
\begin{equation*}
\left( H_{1},\dots,H_{n}\right) \subseteq \ker T_{\left( \mathbf{A,}\nu ,\Bbbk
\right) }.
\end{equation*}%
Now it is sufficient to show that $\ker T_{\left( \mathbf{A,}\nu ,\Bbbk \right)
}\subseteq \left( H_{1},\dots,H_{n}\right) $: Let $g$ be any element of $I$. By
Lemma \ref{lem42} there is unique polynomial $p\in \left\{ f\in \Bbbk \left[
x_{1},\dots,x_{n}\right] :\deg _{i}f<\deg H_{i},i=1,\dots,n\right\} =V\left( 
\mathbf{A,}\nu \right) $ such that 
\begin{equation}\label{43}
g=p+\left( H_{1},\dots,H_{n}\right)  
\end{equation}%
From (\ref{43}) we obtain that for any $\mathbf{m\in }\left[ \mathbf{%
0,}\nu \left( \mathbf{a}\right) -\mathbf{1}\right] $ and any$~\mathbf{a\in A}
$ 
\begin{equation*}
\partial _{\mathbf{a}}^{\mathbf{m}}g=\partial _{\mathbf{a}}^{\mathbf{m}}p,
\end{equation*}%
which implies $\partial _{\mathbf{a}}^{\mathbf{m}}p=0$. Therefore, 
Corollary 2.4 \ yields that $p=0,$ which combined with $\left( 4.3\right) $
gives $g\in \left( H_{1},\dots,H_{n}\right) .$
\end{proof}

\begin{rem}
By Theorem \ref{thm43} it follows that $\left\{ H_{1}\left( x_{1}\right)
,\dots,H_{n}\left( x_{n}\right) \right\} $ is a reduced Gr{\"o}bner basis of $\ker T_{\left( \mathbf{A,}\nu ,\Bbbk \right) }$.
\end{rem}

Given the polynomials $f_{i}\in \Bbbk \left[ x_{i}\right] ,~i=1,\dots,n,$, $A_{i}$, the sets of their roots in the algebraic closure $\overline{\Bbbk }$
of $\Bbbk $, and $\nu _{i}\left( a\right) $ the multiplicity of $a\in A_{i}$, we obtain $f_{i}\left( x_{i}\right) =\prod_{a\in A_{i}}\left( x_{i}-a\right)
^{\nu _{i}\left( a\right) },~i=1,\dots,n$. The ideal of $\overline{\Bbbk }\left[
x_{1},\dots,x_{n}\right] $ is denoted by $\overline{I}$ and it is   generated by $f_{1},\dots,f_{n}$. For $g\in \Bbbk \left[ x_{1},\dots,x_{n}\right] $ let us denote by $\overline{g%
}\ $the residue class of $g$\ in $\overline{\Bbbk }\left[ x_{1},\dots,x_{n}%
\right] /\overline{I}$ .

\begin{cor}\label{cor44}
The ideal $\left( f_{1},\dots,f_{n}\right) $ of $\Bbbk \left[ x_{1},\dots,x_{n}%
\right] $ is equal to $\ker T_{\left( \mathbf{A,}\nu ,\overline{\Bbbk }%
\right) }\cap \Bbbk \left[ x_{1},\dots,x_{n}\right] .$
\end{cor}

\begin{proof}
By Theorem \ref{thm43} we get $\left( f_{1},\dots,f_{n}\right) \subseteq
\ker T_{\left( \mathbf{A,}\nu ,\overline{\Bbbk }\right) }\cap \Bbbk \left[
x_{1},\dots,x_{n}\right] $. Therefore, it is sufficient to prove that $\ker
T_{\left( \mathbf{A,}\nu ,\overline{\Bbbk }\right) }\cap \Bbbk \left[
x_{1},\dots,x_{n}\right] \subseteq \left( f_{1},\dots,f_{n}\right) :$ \ Let $f$
be any element of $J\left( \mathbf{A,}\nu \right) \cap \Bbbk \left[
x_{1},\dots,x_{n}\right] .$ Then by Theorem \ref{thm43} we get
\begin{equation}\label{44}
f=\sum_{i=1}^{n}f_{i}g_{i}, 
\end{equation}%
where $g_{i}\in \overline{\Bbbk }\left[ x_{1},\dots,x_{n}\right]$. Consider
the finite field extension $\Bbbk \subset \Bbbk_{1}$, where $\Bbbk_{1}$ is
the field constructed by adjunction of all coefficients of the polynomials $g_{i}.$ Let $r$ be the degree of $\Bbbk \subset \Bbbk _{1}$ and $\rho $ a
primitive element. Then (\ref{44}) can be written as 
\begin{equation}\label{45}
f=\sum_{j=0}^{r-1}\rho ^{j}\sum_{i=1}^{n}f_{i}g_{ij},  
\end{equation}
where $g_{ij}\in \Bbbk \left[ x_{1},\dots,x_{n}\right]$. Finally, since $
\left\{ 1,\rho ,\dots,\rho ^{r-1}\right\} $ is $\Bbbk$- linearly independent, from (\ref{45}) we obtain
\begin{equation*}
f=\sum_{i=1}^{n}f_{i}g_{i0}.
\end{equation*}%
That is $f\in I.$
\end{proof}

\begin{rem}\label{rem10}
Corollary \ref{cor44} can also be formulated  as: $f\in \left(
f_{1},\dots,f_{n}\right) \subset \Bbbk \left[ x_{1},\dots,x_{n}\right] $, if and
only if $ \partial _{\mathbf{a}}^{\mathbf{m}}f=0,$ for each $\mathbf{a\in A}
$ and$~\mathbf{m\in }\left[ \mathbf{0,}\nu \left( \mathbf{a}\right) -\mathbf{%
1}\right]$.
\end{rem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Let $A_{i},~i=1,\dots,n,$ be finite subsets of an infinite field $\Bbbk $, and $
\nu _{i}\left( a\right) $ the multiplicity of $a\in A_{i}$, and  the
polynomials $H_{i}\left( x_{i}\right) =\prod_{a\in A_{i}}\left(
x_{i}-a\right) ^{\nu _{i}\left( a\right) }\in \Bbbk \left[ x_{i}\right]
,~i=1,\dots,n.$ Given any polynomial $g\in \Bbbk \left[ x_{1},\dots,x_{n}\right] 
$ we apply the Euclidean polynomial division $n$-times.
Assuming that we start with the 1st dimension, there are unique polynomials $q_{1},r_{1}\in \Bbbk \left[
x_{1},\dots,x_{n}\right] $ with $\deg _{1}r_{1}<\deg H_{1}$, such that $%
g=H_{1}q_{1}+r_{1},$. Continuing with the 2nd dimension ($i=2$), there are unique polynomials $q_{2},r_{2}\in \Bbbk %
\left[ x_{1},\dots,x_{n}\right] $ with $\deg _{i}r_{2}<\deg H_{i}$,~$i=1,2~$%
such that $r_{1}=H_{2}q_{2}+r_{2}.$ Continuing in a similar manner until the last dimension, $n$, we obtain unique polynomials $%
q_{n},r_{n}\in \Bbbk \left[ x_{1},\dots,x_{n}\right] $ with $\deg
_{i}r_{n}<\deg H_{i}$,~$i=1,2,\dots,n~$such that $r_{n-1}=H_{n}q_{n}+r_{n}.$
Combining the above $\ n$ polynomial divisions we get 
\begin{equation}\label{rel46}
g=r_{n}+\sum_{i=1}^{n}H_{i}q_{i}.  
\end{equation}

It is easy to verify that for $n$ dimensions there are $n!$ different orders of application of the polynomial divisions, all of which lead to the same result $r_n.$  

\begin{prop}\label{proer1}
Given any polynomial $g\in \Bbbk \left[ x_{1},\dots,x_{n}\right] $, the
interpolating polynomial of the interpolation as presented in Theorem
\ref{thm1} with $t_{\mathbf{a}}^{\mathbf{m}}:=\partial _{\mathbf{a}}^{\mathbf{m}}g,~%
\mathbf{a\in A},~\mathbf{m\in }\left[ \mathbf{0,}\nu \left( \mathbf{a}%
\right) -\mathbf{1}\right] $ is equal to $r_{n}$, and the remainder is equal
to $$\sum_{i=1}^{n}H_{i}q_{i}.$$

\end{prop}


\begin{proof}
From $\deg _{i}r_{n}<\deg H_{i}$,~$i=1,2,\dots,n~$\ we have that $r_{n}\in
V\left( \mathbf{A,}\nu \right) ,$ and from (\ref{rel46}) by Remark \ref{rem10} we obtain $\partial _{\mathbf{a}}^{\mathbf{m}}g=\partial _{\mathbf{a}}^{%
\mathbf{m}}r_{n},~\mathbf{a\in A},~\mathbf{m\in }\left[ \mathbf{0,}\nu
\left( \mathbf{a}\right) -\mathbf{1}\right]$. These arguments in combination
with (\ref{rel46}) lead us immediately to the claims of the current
proposition.
\end{proof}


Proposition \ref{proer1} can be used to express the remainder of the Hermite interpolation in closed form using the cascaded polynomial divisions in case of interpolating a polynomial function. In the general case of any differentiable function to be interpolated (other than polynomial), this error calculation is applicable after expanding the function using Taylor Theorem. The following examples demonstrates error calculation for a univariate and a 3-D polynomial function. 


\begin{exam} \label{hermerrr}
{\rm
Let $g=(x-2)^{11}+x^4+9$. Consider the grid $A=\{0.7, 1.2 ,1.7, 2.2\}$, with multiplicity function $\nu(a) = 2 $, for every point on the grid $a \in A$. We derive the polynomial $H_1(x)= (x-0.7)^2(x-1.2)^2(x-1.7)^2(x-2.2)^2$.
Applying Eq.(\ref{rel46}), we obtain the quotient $q$ and the remainder $r$ of the polynomial division $\frac{g}{H_1}.$
According to Eq.(\ref{rel46}), $r$ is the Hermite polynomial with $\deg r=\sum(a_i)-1=7$, given by


\begin{eqnarray*}
r = \frac{9273}{178} x^7   
    -593 x^6    +      \frac{31499}{11} x^5     -\frac{106481}{14}x^4 +      \frac{108109}{9} x^3      -\frac{349850}{31}x^2    
   +\frac{40932}{7}x -\frac{6409}{5} .
\end{eqnarray*}
The error of the Hermite interpolation is easily obtained by
\begin{eqnarray*}
R &=&H_1 q_1=
x^{11} -22x^{10}   +220x^9  -1320x^8     +\frac{52279}{10}x^7
  -14191x^6 +\frac{293749}{11}x^5 -\frac{173166}{5}x^4 +\frac{272051}{9}x^3\\ &&-\frac{33749}{2}x^2 
   +\frac{37916}{7}x -\frac{3786}{5}.
\end{eqnarray*}


It can be observed that the Hermite polynomial $r(x)$ is unique among the polynomials of degree up to 7 that satisfies the requirements $g(a_i)=r(a_i) \text{ and }\frac{dg}{dx}=\frac{d r}{d x}$ for each supporting point $a_i$. The interpolated function $g(x)$ and the resulting Hermite polynomial are depicted in Figure \ref{hermer} (a). The interpolation error is plotted in the semi-logarithmic graph of Figure \ref{hermer} (b). The error remains very low in $[a_1,a_4]$ and approaches 0 very fast in the vicinity of the $a_i$.


%%%%%%%%%%%%%%%%%%%%%
\begin{exam}
Let us consider $g=(x-2y)^7 +(x+z^2)^4$ and the grid $\mathbf{A}=\{-1, 0 ,1\}\times\{-1, 0 ,1\}\times\{-1, 0 ,1\}$, with multiplicity function $\nu(\mathbf{a}) = (2,2,2) $, for every point on the grid $\mathbf{a} \in \mathbf{A}$. We derive the polynomials $H_1(x)= (x-1)^2(x)^2(x+1)^2$, $H_2(y)= (y+1)^2(y)^2(y+1)^2$ and $H_3(z)= (z+1)^2(z)^2(z+1)^2$.
Applying Eq.(\ref{rel46}), we obtain the quotient $q_1$ and the remainder $r_1$ of the polynomial division $\frac{g}{H_1}.$, Subsequently, we obtain the quotient $q_2$ and the remainder $r_2$ of the polynomial division $\frac{r_1}{H_2}$ and finally, the quotient $q_3$ and the remainder $r_3$ of the polynomial division $\frac{r2}{H_3}.$
According to Eq.(\ref{rel46}), $r_3$ is the Hermite polynomial given by
$$r_3=84x^5y^2 + 2x^5 - 280x^4 y^3 - 28x^4y + 560x^3y^4 - 672x^2y^5 + 14x^2y + 3x^2z^2 + 896x y^4 - 448 x y^2 + 3 x z^4 - 256 y^5 + 128 y^3 + 2 z^4 - z^2$$
The remainder $R=H_1q_1+H_2q_2+H_3q_3$ is calculated as:
$$R=z^2(z^2 - 1)^2 + x^2(x - 14y)(x - 1)^2(x + 1)^2 + y^2(448x - 128y)(y - 1)^2 (y + 1)^2.$$
\end{exam}


%%%%%%%%%%%%%%%%%%%%%%


\begin{figure}[h!]
\centering
\subfigure[]{{\includegraphics[width=0.6\textwidth]{Hermite1D.png}}}\hfill
\subfigure[]{{\includegraphics[width=0.6\textwidth]{Hermite1D_error.png}}}
\caption{
(a) The interpolated function and Hermite polynomial of the Example \ref{hermerrr}, along with the support points  (b) Semi-logarithmic plot of the remainder of interpolation.}
\label{hermer}
\end{figure}

}
\end{exam}





==> rema1.tex <==
\begin{rem}
{\rm
Regarding the computational burden introduced by the calculation of the formula (\ref{mainform}): Let $n$ be the number of dimensions. Consider the grid $\mathbf{A}=A_1 \times \dots \times A_n$, and $N_1=|A_1|,\dots, N_n = |A_n|$ the corresponding cardinalities. Let $k= |v(\mathbf{a})|$, where $v(\mathbf{a})$ is the multiplicity function and $N$ the number of support points, with $N=N_1 \cdot \ldots \cdot N_n$. The computational complexity of $H_{\left( i,a\right) }\left( x_{i}\right)$ in (\ref{Hmikra}), for all $i\in \left\{ 1,\dots,n\right\} $ and $a\in A_{i}$, is
\begin{equation}\label{comp1}
   ((N_1-1)+\dots+(N_n-1))\cdot c_1=(N_1+\dots+N_n -n)k c_1,
\end{equation}
where $c_1$ is a constant factor.

The computational complexity of $H_{(\mathbf{a},\mathbf{k})}$ in (\ref{Hmegala}), for every $\mathbf{a} \in \mathbf{A}$ and $\mathbf{k} \in [\mathbf{0},v(\mathbf{a})-\mathbf{1}]$, is
\begin{equation} \label{comp2}
    N\cdot n \cdot k \cdot c_2,
\end{equation}
where $c_2$ is a constant factor.

The computational complexity introduced by the calculation of inverse of  matrices $\Lambda _{\mathbf{a}} $  in (tade), for every $\mathbf{a} \in \mathbf{A}$ is 
\begin{equation} \label{comp3}
    \left(k^3 + k \cdot n \cdot \left( k^2 - k\right)\right) \cdot N \cdot c_3,
\end{equation}
where $c_3$ is a constant factor.

The matrix multiplications done in (\ref{mainform}) have computational complexity 
\begin{equation} \label{comp4}
    N \cdot k^2 \cdot c_4,
\end{equation}
where $c_4$ is a constant factor.

Combining (\ref{comp1}), (\ref{comp2}), (\ref{comp3}), and (\ref{comp4}), the resulting complexity is 
\begin{equation}\label{compl_ours}
    \left(N_1+\dots+N_n -n\right) \cdot k \cdot c_1 + N\cdot n \cdot k \cdot c_2 +\left(k^3 + k \cdot n \cdot \left( k^2 - k\right)\right) \cdot N \cdot c_3 +N\cdot k^2\cdot c_4 = O(k^3 \cdot n \cdot N).
\end{equation}

Regarding the computational complexity resulting from the closed form expression in  \cite[Theorem 4.2]{fractmult}: The computational burden of calculating all  $ H_{a_j}(x_j)$ and $G_{a_{j}}^{k_{j}}$ is
\begin{equation*}
    (N_1+\cdots +N_n -n)\cdot k+ N\cdot k^2\cdot c_5,
\end{equation*}
and the resulting complexity in order to compute (\ref{ndpolmeh}) is 
\begin{equation}\label{compl_Pandey}
N_1+\cdots +N_n -n + N^2 \cdot k^{n+2} \cdot n \cdot c_6 = O(N^2 \cdot k^{n+2} \cdot n).
\end{equation}
where $c_5,c_6$ are  constant factors.

It becomes obvious that the computational complexity of the Hermit interpolant in the form of \cite[Theorem 4.2]{fractmult} is not polynomial with respect to $k$, whereas the complexity of the proposed Hermite interpolant is of polynomial time with respect to $k$. }
%It is also worth mentioning that the polynomials $G^{k}_{a}$ in (\ref{polspy}) have maximum degree $\nu_{i}(a) \cdot (n-1) + \nu_{i}(a) -k -1 +$, whereas the maximum degree is $\nu_{i}(a) \cdot (n-1) + \nu_{i}(a) -k -1$
\end{rem}

==> splinecontinunity.tex <==
\textcolor{black}{
In this subsection, we provide formal proof that the proposed Hermite polynomials form a continuous spline. To this end, we will consider two $n$-dimensional grids, $\mathbf{A}_{a-}^{k}$ and $\mathbf{A}_{a+}^{k}$, which share a common hyperplane of support points normal to the $k^{th}$ dimension at position $a_k=a$. It will suffice to prove that the two correspondingly defined polynomials are continuous along the common hyperplane.
}

\textcolor{black}{
More formally, let $A_{i},~i=1,\dots,n$, be finite subsets of $
\mathbb{R}$, and $\nu _{i}\left( a\right) $ be the multiplicity of $a\in {A_i}$, and finally $\ t_{\mathbf{a}}^{\mathbf{k}}\in \Bbbk \,,~\mathbf{a\in A},$ $\mathbf{k\in }\left[ 
\mathbf{0,}\nu \left( \mathbf{a}\right) -\mathbf{1}\right]$. Consider the
polynomials $H_{i}\left( x_{i}\right) =\prod_{a\in A_{i}}\left(
x_{i}-a\right) ^{\nu _{i}\left( a\right) }\in \Bbbk \left[ x_{i}\right]
,~i=1,\dots,n$. Further for any $k=1,\dots,n$, any $a\in A_{k},$ 
let us denote $\mathbf{A}_{a-}^{k}:=\left\{ \mathbf{a\in A:}\text{ }a_{k}\leq a\right\} $, $%
\mathbf{A}_{a+}^{k}:=\left\{ \mathbf{a\in A:}\text{ }a_{k}\geq a\right\} $,
and $\mathbf{A}_{a}^{k}:=\left\{ \mathbf{a\in A:}\text{ }a_{k}=a\right\} .$
Clearly the following is valid $\mathbf{A}_{a-}^{k}\cap \mathbf{A}_{a+}^{k}=\mathbf{A}%
_{a}^{k}$. Consider the vector spaces $V\left( \mathbf{A}_{a-}^{k}\mathbf{,}%
\nu \right) $, $V\left( \mathbf{A}_{a+}^{k}\mathbf{,}\nu \right) \,$as
defined in the introduction and the vector space $V\left( \mathbf{A}_{a}^{k}%
\mathbf{,}\nu \right) $ consisting of all polynomials $f\left(
x_{1},\dots,x_{k-1},a,x_{k+1}\dots,.,x_{n}\right) $, such that $\deg
_{i}f<\sum_{a\in A_{i}}\nu _{i}\,\left( a\right) ,i=1,\dots,k-1,k+1,\dots,n.$ We
denote by $p_{a-}^{k}$ and $\ p_{a+}^{k}$  the following two unique Hermite interpolant polynomials (see Theorem
\ref{thm1}) of the vector spaces $V\left( \mathbf{A}_{a-}^{k}%
\mathbf{,}\nu \right) $ and $V\left( \mathbf{A}_{a+}^{k}\mathbf{,}\nu
\right) $ respectively, which satisfy the following conditions:%
\begin{equation}\label{eqtaged1}
\partial _{\mathbf{a}}^{\mathbf{m}}p_{a-}^{k}=t_{\mathbf{a}}^{\mathbf{m}},~%
\mathbf{a\in A}_{a-}^{k},~\mathbf{m\in }\left[ \mathbf{0,}\nu \left( \mathbf{%
a}\right) -\mathbf{1}\right],   
\end{equation}%
and 
\begin{equation}\label{eqtaged2}
\partial _{\mathbf{a}}^{\mathbf{m}}p_{a+}^{k}=t_{\mathbf{a}}^{\mathbf{m}},~%
\mathbf{a\in A}_{a+}^{k},~\mathbf{m\in }\left[ \mathbf{0,}\nu \left( \mathbf{%
a}\right) -\mathbf{1}\right] . 
\end{equation}
} 

\begin{thm}
\textcolor{black}{
    The Hermite polynomials $\left\{ 
\begin{array}{cc}
p_{a-}^{k}\left( \mathbf{x}\right) , & \mathbf{x\in A}_{a-}^{i} \\ 
p_{a+}^{k}\left( \mathbf{x}\right) , & \mathbf{x\in A}_{a+}^{i}%
\end{array}%
\right. $ form a continuous spline for any $\mathbf{x}$ with $x_k=a$.
}
\end{thm}
 

\begin{proof}
\textcolor{black}{
It is sufficient to prove the following identity: 
$$
p_{a-}^{k}\left( x_{1},\dots,x_{k-1},a,x_{k-1},\dots,x_{n}\right)
=p_{a+}^{k}\left( x_{1},\dots,x_{k-1},a,x_{k-1},\dots,x_{n}\right). 
$$
Given $p_{a-}^{k}\in V\left( \mathbf{A}_{a-}^{k}\mathbf{,}\nu \right) $, and $%
p_{a+}^{k}\in V\left( \mathbf{A}_{a+}^{k}\mathbf{,}\nu \right) $ it holds that  
$$
p_{a-}^{k}\left( x_{1},\dots,x_{k-1},a,x_{k-1},\dots,x_{n}\right), $$ and 
$$
p_{a+}^{k}\left( x_{1},\dots,x_{k-1},a,x_{k-1},\dots,x_{n}\right) $$ are elements
of the vector space $V\left( \mathbf{A}_{a}^{k}\mathbf{,}\nu \right)$. Therefore the
polynomial $$p:=p_{a-}^{k}\left( x_{1},\dots,x_{k-1},a,x_{k-1},\dots,x_{n}\right)
-p_{a+}^{k}\left( x_{1},\dots,x_{k-1},a,x_{k-1},\dots,x_{n}\right) $$ 
is also an element of $V\left( \mathbf{A}_{a}^{k}\mathbf{,}\nu \right) .$ 
By  (\ref{eqtaged1}) and (\ref{eqtaged2}), for  $~\mathbf{a\in A}_{a}^{k},~%
\mathbf{m\in }\left[ \mathbf{0,}\left( \nu \left( a_{1}\right) ,\dots,\nu
\left( a_{k-1}\right) ,1,\nu \left( a_{k+1}\right) ,\dots,\nu \left(
a_{n}\right) \right) -\mathbf{1}\right] $, we get   $$\partial
_{a_{1}}^{m_{1}}\dots\partial _{a_{k-1}}^{m_{k-1}}\partial
_{a_{k+1}}^{m_{k+1}}\dots\partial _{a_{n}}^{m_{n}}p\left(
x_{1},\dots,x_{k-1},a,x_{k-1},\dots,x_{n}\right) =0.$$ Therefore by Corollary \ref{cor24}, it
follows $p=0.$ 
}
\end{proof}
\textcolor{black}{
Since, after substitution $x_k=a$, the two polynomials $p_{a-}^k$, $p_{a+}^k$ are identical, it follows that their derivatives are also continuous.
Considering the above and Theorem \ref{thm1} about the uniqueness of Hermite interpolation polynomial, it follows that the proposed Hermite spline is regular}. 

\begin{exam} \label{examplesplinecont}
{\rm 
\textcolor{black}{
Let us demonstrate the continuity of the proposed Hermite spline by constructing two Hermite interpolants each one generated by $2 \times 2$ support points on the $\mathbb{R}^2$ plane, while sharing two of these support points. More specifically, let $A_1=\{0,1,2\}$ and $A_2=\{0,1\}$. Then $\mathbf{A}=A_1 \times A_2$. Following the formalism of subsection \ref{contsplines}, we select the support points with $a=1$  (along the $1^{st}$ dimension: $k=1$). Thus, $\mathbf{A}_{1^-}^1=\{0,1\} \times \{0,1\}$  are the support points of Hermite polynomial $p_{1-}^{1}$ and $\mathbf{A}_{a+}^{1} =\{1,2\} \times \{0,1\}$ are the support points of Hermite polynomial $p_{1+}^{1}$. Clearly, the common support points are given by $\mathbf{A}_{a-}^{k}\cap \mathbf{A}_{a+}^{k}=\mathbf{A}_{a}^{k}$, which in this example are just two points: $(1,0)$ and $(1,1)$ both with $x_1$ coordinate equal to 1. The multiplicity function is set for all points as $\nu(\mathbf{a})=3$, for all $\mathbf{a}$.
According to  Theorem \ref{finterpform} the two Hermite interpolants are given by the formulas:
} 
$p_{1-}^{1}(x_1,x_2)=-\left(-5\,{x_{2}}^2+x_{2}+1\right)\,\left({x_{1}}^3-2\,{x_{1}}^2+3\,x_{1}-4\right)$, 

$p_{1+}^{1}(x_1,x_2)=-4.2516\,{x_{1}}^5\,{x_{2}}^5+11.7596\,{x_{1}}^5\,{x_{2}}^4-8.6201\,{x_{1}}^5\,{x_{2}}^3+24.9583\,{x_{1}}^5\,{x_{2}}^2-2.5212\,{x_{1}}^5\,x_{2}-5.2075\,{x_{1}}^5+30.9691\,{x_{1}}^4\,{x_{2}}^5-86.0186\,{x_{1}}^4\,{x_{2}}^4+63.3642\,{x_{1}}^4\,{x_{2}}^3-179.7732\,{x_{1}}^4\,{x_{2}}^2+17.3778\,{x_{1}}^4\,x_{2}+37.5189\,{x_{1}}^4-87.3513\,{x_{1}}^3\,{x_{2}}^5+243.6424\,{x_{1}}^3\,{x_{2}}^4-180.4411\,{x_{1}}^3\,{x_{2}}^3+494.6803\,{x_{1}}^3\,{x_{2}}^2-45.0001\,{x_{1}}^3\,x_{2}-103.1784\,{x_{1}}^3+118.7548\,{x_{1}}^2\,{x_{2}}^5-332.4123\,{x_{1}}^2\,{x_{2}}^4+247.3391\,{x_{1}}^2\,{x_{2}}^3-649.9843\,{x_{1}}^2\,{x_{2}}^2+54.9454\,{x_{1}}^2\,x_{2}+135.4968\,{x_{1}}^2-78.0744\,x_{1}\,{x_{2}}^5+219.1735\,x_{1}\,{x_{2}}^4-163.7111\,x_{1}\,{x_{2}}^3+420.2292\,x_{1}\,{x_{2}}^2-33.7958\,x_{1}\,x_{2}-87.4964\,x_{1}+19.9533\,{x_{2}}^5-56.1446\,{x_{2}}^4+42.0691\,{x_{2}}^3-120.1103\,{x_{2}}^2+10.9939\,x_{2}+24.8667$

\textcolor{black}{
Figure \ref{figsplincont2d} shows $p_{1-}^{1}(x_1,x_2)$ and $p_{1+}^{1}(x_1,x_2)$ in blue and green color respectively.
By substituting $x_1 = 1$ in $p_{1-}^{1}, p_{1+}^{1}$ we get 
\begin{eqnarray*}
    p_{1-}^{1} = -10x_2^2+ 2 x_2 +2, \;\;\;p_{1+}^{1}(x_2)= -10x_2^2+ 2 x_2 +2,
\end{eqnarray*}
which confirms the continuity of the two polynomials and their derivatives.
}


\begin{figure}[!h]
     \centering
         \includegraphics[width=9cm]{continuity_example2D.png}
         \caption{The two Hermite interpolants of example \ref{examplesplinecont} with the support points shown as red circles. The continuity of the Hermite spline along the points with $x_1=1$ is visually confirmed.}
         \label{figsplincont2d}
\end{figure}
}
\end{exam}


==> splinsection.tex <==
In our recent work \cite{DK23} we established the $n$-dimensional Hermite spline and proved its continuity. To briefly summarize the properties of the proposed Hermite splines, they were defined for even, as well as odd number of local support points, which is also referred as stencil. The maximum degree of each of the univariate Hermite polynomials for each dimension is given by the following formula:
\begin{equation}
    %\max_{a\in A_i}\{v_i(a)\} -\min_{a\in A_i}\{v_i(a)\}- 1 + \sum_{a \in A_i} v_i(a) =
     \max_{a\in A_i}\min_{b \in A_i}\{v_i(a)-v_i(b)\} - 1 +  \sum_{a \in A_i} v_i(a).
\end{equation}

The maximum total degree of the polynomial is:
\begin{equation}
   \sum_{i=1}^{n}\left(\max_{a\in A_i}\min_{b \in A_i}\{v_i(a)-v_i(b)\} - 1 +  \sum_{a \in A_i} v_i(a) \right)
\end{equation}
 


 
The local support points along the $i^{\text{th}}$ dimension can be defined as follows. In the case of even $|B|$ the local support points along the $i$ dimension a defined as the closest $\frac{|B|}{2}$ points less than $q_i$ and the $\frac{|B|}{2}$ points closest and greater than $q_i$. 
In the case of odd $|B|$, the local support points along the $i$ dimension are defined as the single support point with $ith$ coordinate closest to $q_i$, and the $\frac{|B|- 1}{2}$ support points less than the closest and the $\frac{|B|- 1}{2}$ support points with $ith$ coordinate greater than the closest support point. 
In the most common case, where the Hermite interpolation is applied to signals in one or more dimensions, the support points are assumed to have integer coordinates, and the local support points are defined as follows:

\begin{equation}
   B_i:= \begin{cases}
     \left[ [q_{i}] -\frac{|B_i|-1}{2}, \dots, [q_{i}] +\frac{|B_i|-1}{2}\right]&,  \; \text{if }n\; |B_i|\mod 2=1 \\
     &\\
     \left[ \lfloor q_{i} \rfloor {-\frac{|B_i|}{2}+1}, \dots, \lfloor q_{i} \rfloor +\frac{|B_i|}{2}\right]&,  \; \text{otherwise}
   \end{cases}, \;i=1,\dots, n,
   \label{spline_local_sup}
\end{equation}
where $\lfloor .\rfloor$ denotes the rounding to the smallest nearest integer (floor) operator and $[.]$ denotes the rounding to the nearest integer (round) operator.
Fig. \ref{figsplinevis2d} and %\ref{figsplinevis3d} 
visualize the support points for a random point $\mathbf{q}$ denoted by the green circle and $\lvert B_1 \rvert=\lvert B_2 \rvert=3$ in 2D and $\lvert B_1 \rvert=\lvert B_3 \rvert=\lvert B_3 \rvert=3$ in 3D, respectively, according to Eq.(\ref{figsplinevis2d}).
%3,4 masks 


\begin{figure}[!ht]
     \centering
  \includegraphics[width=9cm]{2dspline.png}
         \caption{Visualization of an example of spline local support points round a random point (green circle) in 2D, with $\lvert B_1 \rvert=\lvert B_2 \rvert=3$. }
         \label{figsplinevis2d}
\end{figure}

\begin{comment}

\begin{figure}[!h]
     \centering
         \includegraphics[width=12cm]{3dspline.png}
         \caption{Visualization of an example of spline local support points round a random point (green circle) in 3D, with $\lvert B_1 \rvert=\lvert B_2 \rvert=\lvert B_3 \rvert=3$. }
         \label{figsplinevis3d}
\end{figure}
    
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 


\begin{comment}

\subsection{Continuity of the proposed Hermite Splines}
\label{contsplines}
\input{splinecontinunity}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
 
\textcolor{black}{In the example below we provide a univariate example to further facilitate the continuity demonstration. More specifically we generate a univariate Hermite spline over $7$ support points for each Hermite interpolant, using $4$ local support points, for different values of the multiplicity function $v(a)=1,2,3$. The continuity of the interpolants and their derivative can be visually confirmed.}



\begin{exam} \label{exxxx}
{\rm
\textcolor{black}{
Consider the grid $A=\{0,\dots ,6\}$ and the Hermite polynomial $f(x)$ which satisfies $\partial _{{a}}^{{m}}f=t_{{a}}^{{m}}, 
{a\in A}$, ${m\in }\left[ {0,}\nu \left( {a}%
\right) -1\right]$ with known values given in Table \ref{tablyexxx}.
For any $x \in [0,6]$ we derive the spline Hermite polynomial, defined in $\Big[\lfloor x \rfloor, \lceil x \rceil \Big]$, using $|B|=4$ number of local support points, with $B=\Big[\lfloor x \rfloor -1, \lceil x \rceil +1 \Big]$
%Let $g=(x-2)^8 - (x+3)^4 +(x-7)^3+7 x^2+8$,
for different values of the multiplicity function $\nu(a) = \{1,2,3\} $ and for every point $a$ on the grid $ A$. In Fig. \ref{fisubfigxx}(a) the spline Hermite polynomials are shown in different colors for each domain, whereas the style of the line indicates the value of $\nu(a)$, as follows: dotted line: $\nu(a)=1$, dashed line: $\nu(a)=2$ and continuous line: $\nu(a)=3$. 
The 1st, 2nd, and 3rd derivatives of the spline Hermite polynomials are shown in Fig.  \ref{fisubfigxx}(b), (c), and (d), respectively. As was expected, the Hermite spline is continuous ($C^0$) for all values of $\nu(a)>0$, the 1st derivative of the Hermite spline is continuous ($C^1$) for $\nu(a)=\{2,3\}$, the 2nd derivative is continuous ($C^2$) only for $\nu(a)=3$.}


\begin{table}[!h]
\begin{center}
\caption{The conditions that must be satisfied by the Hermite polynomial in Example  \ref{exxxx}}\label{tablyexxx}
\begin{tabular}{|l ccc|}
\hline
$\mathbf{a}$ & $t^0_{{a}}$ & $t^1_{{a}}$ & $t^2_{{a}}$\\ \hline
0 &  -160 & -985 & 3448\\ \hline
1  &  -456  &  -142 & -158\\ \hline
2 &  -714 &  -397 & -316 \\ \hline
3 &  -1288 &  -766 & -386 \\ \hline
4 & -2052 &   -265 & 2992\\ \hline
5   & 2640 &  15530 & 40058\\ \hline  
6  &  59234 & 128243 & 228412\\ \hline
\hline
\end{tabular}
\end{center} 
\end{table}


\begin{figure}[h!]
\centering
\subfigure[]{{\includegraphics[width=0.5\textwidth]{C0.png}}}\hfill
\subfigure[]{{\includegraphics[width=0.5\textwidth]{C1.png}}}
\subfigure[]{{\includegraphics[width=0.5\textwidth]{C2.png}}}\hfill
\subfigure[]{{\includegraphics[width=0.5\textwidth]{C3.png}}}
\caption{\textcolor{black}{The continuity of the interpolants of $f(x)$, with multiplicity functions $\nu(a) = \{1,2,3\} $, for every point $a$ on the grid $ A$,  and its derivatives up to order 3 of Example \ref{exxxx}. The different colors indicate the different spline interpolants for each interval. Dotted, dashed and continuous line indicates the interpolant created with $v(a)=1$, $v(a)=2$ and $v(a)=3$, respectively.  (a) the $C^0$ continuity of the spline interpolants $f(x)$ (b) $C^1$ continuity of the spline interpolants of $f(x)$ (c) the $C^2$ continuity of the spline interpolants of $f(x)$ (d) the $C^3$ continuity of the spline interpolants of $f(x)$}.}
\label{fisubfigxx}
\end{figure}



}
\end{exam}
    
\end{comment}
